Cache-Assisted Broadcast-Relay Wireless Networks: A Delivery-Time Cache-Memory Tradeoff

An emerging trend of next generation communication systems is to provide network edges with additional capabilities such as storage resources in the form of caches to reduce file delivery latency. To investigate this aspect, we study the fundamental limits of a cache-aided broadcast-relay wireless network consisting of one central base station, $M$ cache-equipped transceivers and $K$ receivers from a latency-centric perspective. We use the normalized delivery time (NDT) to capture the per-bit latency for the worst-case file request pattern, normalized with respect to a reference interference-free system with unlimited transceiver cache capabilities. The objective is to design the schemes for cache placement and file delivery in order to minimize the NDT. To this end, we establish a novel converse and two types of achievability schemes applicable to both time-variant and invariant channels. The first scheme is a general one-shot scheme for any $M$ and $K$ that synergistically exploits both multicasting (coded) caching and distributed zero-forcing opportunities. We show that the proposed one-shot scheme (i) attains gains attributed to both individual and collective transceiver caches (ii) is NDT-optimal for various parameter settings, particularly at higher cache sizes. The second scheme, on the other hand, designs beamformers to facilitate both subspace interference alignment and zero-forcing at lower cache sizes. Exploiting both schemes, we are able to characterize for various special cases of $M$ and $K$ which satisfy $K+M\leq 4$ the optimal tradeoff between cache storage and latency. The tradeoff illustrates that the NDT is the preferred choice to capture the latency of a system rather than the commonly used sum degrees-of-freedom (DoF). In fact, our optimal tradeoff refutes the popular belief that increasing cache sizes translates to increasing the achievable sum DoF.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Communications Society subset of the full
IEEEtran package and is intended for use with IEEE Communications Society
publications. The included version of the IEEEtran_HOWTO.pdf has been
specially formatted in IEEE Communications Society (comsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf,
                   bare_jrnl_comsoc.tex.
***************************************************************************


==> content/ach__Anas_Chaaban_s_conflicted_copy_2017-12-28_.tex <==
\section{NDT-Optimal Schemes for Special Instances: Combining Subspace Alignment, Multicasting and Zero-Forcing}
\label{sec:ach_special}

In this section, we present our novel achievability scheme that combines the well-known schemes -- interference alignment, multicasting and zero-forcing -- for special instances of $M=\{1,2,3\}$ and $K=\{1,2,3\}$ that satisfy $K+M\leq 4$. For these special instances, this scheme allows us to fully characterize the optimal NDT cache-memory tradeoff for any $\mu\in[0,1]$. 
  
Before establishing the achievability at fractional cache sizes in the range $\mu\in(0,1)$, we consider two special corner points at fractional cache sizes $\mu=0$ and $\mu=1$ for \emph{arbitrary} $M$ and $K$. These are the cases where the RN has either \emph{zero-cache} ($\mu=0$) or \emph{full-cache} ($\mu=1$) capabilities. In the following lemma, we expound the optimal NDT for these two points.  
\vspace{.5em}
\begin{lemma}\label{corr_mu_0_and_1}
	For the transceiver cache-aided network with one DeNB, $M$ RNs each endowed with a cache of fractional cache size $\mu$, $K$ UEs and a file library of $N\geq M+K$ files, the optimal NDT is
	\begin{equation}\label{eq:opt_NDT_mu_0}
	\delta^{\star}(\mu)=K+M\:\:\text{ for }\mu=0,
	\end{equation} 
	achievable via DeNB broadcasting to $M$ RNs and $K$ UEs, and 
	\begin{equation}
	\label{eq:opt_NDT_mu_1}
	\delta^{\star}(\mu)=\max\Bigg\{1,\frac{K}{M+1}\Bigg\}\:\:\text{ for }\mu=1,
	\end{equation} 
	achievable via zero-forcing beamforming for an $(M+1,K)$ MISO\footnote{In MISO broadcast channels, we use the notation, $(a,b)$ for integers $a$ and $b$ to denote a broadcast channel with $a$ transmit antennas and $b$ single antenna receivers.} broadcast channel. 
\end{lemma}

\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.475\textwidth}
		\centering
		\begin{tikzpicture}[scale=0.8]
		\PlotNDTMOneKOne
		\end{tikzpicture}
		\caption[NDT for $M=K=1$]{\small NDT for $M=K=1$}
		\label{fig:NDT_M_K_1_1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.475\textwidth}  
		\centering 
		\begin{tikzpicture}[scale=0.8]
		\PlotNDTMOneKTwo
		\end{tikzpicture}
		\caption[NDT for $M=1,K=2$]{\small NDT for $M=1, K=2$} 
		\label{fig:NDT_M_K_1_2}       
	\end{subfigure}
	\caption[NDT as a function of $\mu$ for $M=1$ and $K\leq 2$]
	{\small Optimal NDT as a function of $\mu$ for $M=1$ and $K\leq 2$} 
	\label{fig:NDT_M_K_1_LEQ_2}
\end{figure*} 


\begin{proof}
	For the proof, it suffices to find a cache transmission policy that matches the lower bound in Thoerem \ref{theorem_lower_bound} for $\mu=0$ and $\mu=1$, respectively. On the one hand, if $\mu=0$, we note that $\delta_{\text{LB}}(0,M,1)=K+M$. On the other hand, if $\mu=1$, we observe that $\delta_{\text{LB}}(1,0,M+1)=\nicefrac{K}{(M+1)}$ if $M+1\leq K$ and $\delta_{\text{LB}}(1,\ell,s)<1$ if $M+1>K$. Next, we consider the achievability at $\mu=0$ and $\mu=1$. For these two fractional cache sizes, the network in Fig. \ref{fig:HetNet} reduces to a SISO broadcast channel (BC) with $K+M$ users for $\mu=0$ and an $(M+1,K)$ MISO broadcast channel for $\mu=1$. The approximate \emph{per-user} rate (neglecting $o(\log(P))$ bits) for these two channels are known to be $\frac{1}{(K+M)}\log(P)$ (achievable through unicasting each user's message) and $\frac{1}{K}\min\{M+1,K\}\log(P)$ (achievable through zero-forcing beamfoming), respectively. Equivalently, each user needs the reciprocal per-user rate of signaling dimensions (e.g., channel uses in time or frequency) to retrieve one desired bit. Thus, the approximate DTB becomes, respectively, $\frac{(K+M)}{\log(P)}$ and $\frac{K}{\min\{M+1,K\}\log(P)}$. Normalizing the delivery time per bit by the point-to-point reference DTB $\frac{1}{\log(P)}$ generates the NDTs $K+M$ and $\max\{1,\nicefrac{K}{(M+1)}\}$. This establishes the NDT-optimality at these fractional cache sizes.
\end{proof}
\vspace{.5em}
\begin{remark}
	From Lemma \ref{corr_mu_0_and_1}, we infer that the caching problem for the system illustrated in Fig. \ref{fig:HetNet} establishes the behavior of the network in terms of delivery time between the two extremes -- SISO BC with $K+M$ users and an $(M+1,K)$ MISO BC. This analysis will reveal what kind of schemes other than simple unicasting and zero-forcing will be optimal for $0<\mu<1$.
\end{remark}
\vspace{.5em}
Now, we move to the aforementioned special cases of the system, where $M=\{1,2,3\}$, to provide a \emph{complete} characterization of the NDT-memory trade-off. We start with the case where $M=1$.  

\subsection{Achievability for $M=1$}\label{subsec:ach_M1}

The NDT-optimal scheme for $M=1$ and $K\leq 3$ is presented. Hereby, the following proposition quantifies the achievable NDT. 

\begin{proposition}\label{prop_M1}
	The achievable NDT of the network under study for $M=1$ RNs, $K=\{1,2,3\}$ UEs and $\mu\in[0,1]$ is given by 
	\begin{equation}
	\label{eq:ach_NDT_M_1_K_123}
	\delta(\mu)=\begin{cases}K+1-\mu K\quad&\text{ if } K\leq 2\\\max\bigg\{K+1-\mu K,\frac{K+1-\mu}{2}\bigg\}\quad&\text{ if }K=3\end{cases}.
	\end{equation}
\end{proposition}
In what follows the proof of this proposition is outlined. As shown in Fig. \ref{fig:NDT_M_K_1_LEQ_2}, in the case, where $K\leq 2$, the lower bound $\delta_{\text{LB}}(\mu,\ell=1,s=1)$ coincides with the achievable NDT. Lemma \ref{corr_mu_0_and_1} establishes the achievability for the corner points (marked by circles in Fig. \ref{fig:NDT_M_K_1_LEQ_2}) at $\mu=0$ and $\mu=1$. Hereby, due to arguments of \emph{memory sharing}, intermediary points at fractional cache sizes $0<\mu<1$ become achievable through successively  time-sharing between unicasting and zero-forcing for $\mu$ and $(1-\mu)$ time fractions, respectively.

\begin{figure}
	\centering
	\begin{tikzpicture}[scale=1]
	\PlotNDTMOneKGreatTwo
	\end{tikzpicture}
	\caption[NDT lower bound for $M=1$ and $K\geq 3$]{\small The NDT lower bound for $M=1$ and $K\geq 3$ is shown by the solid line. For $K=3$, this line is in fact achievable. The dashed line shows the achievable NDT of a time-sharing based unicasting-zero-forcing scheme.} 
	\label{fig:NDT_M_K_1_3}
\end{figure}   

However, for $K=3$ such type of memory sharing scheme is in fact \emph{suboptimal} (as shown by the dashed line of Fig. \ref{fig:NDT_M_K_1_3}). Instead we will show that \emph{simultaneously} combining (subspace) alignment with zero-forcing through appropriate precoder design allows us to show the achievability of the corner point $\Big(\frac{K+1}{2K-1},\frac{K^{2}-1}{2K-1}\Big)=\Big(\frac{4}{5},\frac{8}{5}\Big)$ for $K=3$. To this end, we describe, respectively, \begin{enumerate*}[label=(\roman*)]
	\item the \emph{RN cache placement} for $\mu=\nicefrac{4}{5}$,
	\item the \emph{encoding} at DeNB and RN ($M=1$),
	\item and finally the \emph{decoding} at RN and the three UEs ($K=3$).
\end{enumerate*} We begin with the cache placement.  
\vspace{.5em}
\subsubsection*{RN Cache Placement}

\begin{figure}
	\FilesKThree
	\caption[Requested files by $K=3$ users and $M=1$ RNs]{\small Requested files by $K=3$ users and $M=1$ RNs and the availability illustrated by the symbols transmitted from the DeNB only or from both at the DeNB and the RN.}
	\label{fig:files_K_three}
\end{figure}
Assume without loss of generality $N=4$ and that the UEs request files $W_1,W_2$ and $W_3$ while the RN is interested in file $W_4$. According to Fig. \ref{fig:files_K_three}, all files are comprised of $5$ symbols, i.e., the $i$-th file is composed of symbols $\eta_{i,1},\eta_{i,2},\eta_{i,3},\eta_{i,4}$ and $\eta_{i,5}$. \emph{All} these symbols are available at the DeNB. However, as far as the RN is concerned, only the first four symbols of all files are locally available in its cache. Since, the RN is interested in file $W_4$ and it knows $\eta_{4,1},\eta_{4,2},\eta_{4,3}$ and $\eta_{4,4}$, the only missing symbol it desires is $\eta_{4,5}$. Thus, the transmission policy has to be designed such that DeNB and RN are involved in sending \emph{all} symbols of files $W_1,W_2$ and $W_3$ as well as $\eta_{4,5}$. These are in total $16$ information symbols. Next, we describe the encoding strategy for both DeNB and RN. 

\vspace{.5em}
\subsubsection*{Encoding at DeNB and RN}

\begin{figure}[h]
	\ZFKThree
	\caption[Zero-forcing map]{\small Map that assigns which symbol to zero-force at which UE.} 
	\label{fig:ZF_K_three}
\end{figure} 

The transmission strategy will exploit the correlation that arises between the availability of shared symbols at RN and DeNB by leveraging zero-forcing (ZF) opportunities while \emph{simultaneously} facilitating (subspace) interference alignment (IA) at the UEs. This is why our scheme (as shown in Fig. \ref{fig:files_K_three}) only zero-forces symbols $\eta_{1,1},\eta_{1,2},\eta_{1,3}$, $\eta_{2,1},\eta_{2,2},\eta_{2,3}$ and $\eta_{3,1},\eta_{3,2},\eta_{3,3}$. Symbols $\eta_{1,4},\eta_{2,4}$ and $\eta_{3,4}$ are \emph{not} zero-forced but are instead used to enable alignment\footnote{IA is facilitated by the fact that the DeNB does \emph{not} transmit these symbols (even though it knows them). Thus, effectively, the DeNB does not need to be aware of $\eta_{i,4},i\in[N]$.} amongst others with $\eta_{4,5}$ at the UEs. The map that assigns which symbol is zero-forced at which UE is given in Figure \ref{fig:ZF_K_three}. To this end, DeNB and RN form their transmit signals according to 
\begin{align}
\label{eq:tx_sig_DeNB}
x_s[t]&=\sum_{i=1}^{3}\sum_{\substack{j=1,\\j\neq 4}}^{5}\nu_{\eta_{i,j}}[t]\eta_{i,j}+\nu_{\eta_{4,5}}[t]\eta_{4,5},\\
\label{eq:tx_sig_RN}
x_r[t]&=\sum_{i=1}^{3}\sum_{j=1}^{4}\beta_{\eta_{i,j}}[t]\eta_{i,j},
\end{align} $\forall t\in[T]$ for $T=8$, respectively. The complex scalars $\nu_{\eta_{i,j}}[t]$ and $\beta_{\eta_{i,j}}[t]$ are precoders for symbol $\eta_{i,j}$ originating from DeNB and RN at time instant $t$, respectively. They are chosen such that both ZF and IA at the UEs become feasible. According to the ZF map of Fig. \ref{fig:ZF_K_three}, the ZF conditions at UE$_k$, $k\in[K]=[3]$, become \begin{subequations}\label{eq:ZF_conditions}
	\begin{align}
	&\nu_{\eta_{(k+1)\Mod{K},1}}[t]g_k[t]+\beta_{\eta_{(k+1)\Mod{K},1}}[t]h_{k1}[t]=0,\\
	&\nu_{\eta_{(k+1)\Mod{K},2}}[t]g_k[t]+\beta_{\eta_{(k+1)\Mod{K},2}}[t]h_{k1}[t]=0,\\
	&\nu_{\eta_{(k+2)\Mod{K},3}}[t]g_k[t]+\beta_{\eta_{(k+2)\Mod{K},3}}[t]h_{k1}[t]=0.
	\end{align}
\end{subequations} Simultaneously, we design the precoding scalars such that the interference at each UE is aligned into a three-dimensional signal space. (The remaining $5$ dimensions are reserved for the $5$ symbols of the desired file.) The interference graph in Fig. \ref{fig:IA_Graph} shows which symbols align with each other at which UE. This graph consists of $3$ layers. In the first layer, two symbols, namely $\eta_{4,5}$ and $\eta_{1,4}$, $\eta_{2,4}$ or $\eta_{3,4}$ align at the three UEs. At layers two and three, on the other hand, three symbols align per UE. Symbols $\eta_{1,4},\eta_{2,4}$ and $\eta_{3,4}$ link layers $1$ and $2$, while $\eta_{1,5},\eta_{2,5}$ and $\eta_{3,5}$ connect layers $2$ and $3$. In analogy to the graph in Fig. \ref{fig:IA_Graph}, the alignment conditions at UE$_k$ can be written as 
\begin{figure*}[h]
	\centering
	\begin{tikzpicture}[scale=1]
	\AlignGraph
	\end{tikzpicture}
	\caption[Interference Alignment Graph for the achievability at corner point $(\frac{4}{5},\frac{8}{5})$ for $M=1$ and $K=3$]{\small Interference Alignment Graph for the achievability at corner point $(\frac{4}{5},\frac{8}{5})$ for $M=1$ and $K=3$. The graph consists of three (subspace) alignment chains. By definition, the first alignment chain is the path from the node $\eta_{4,5}$ to $\eta_{3,1}$, the second from $\eta_{4,5}$ to $\eta_{1,1}$ and the third from $\eta_{4,5}$ to $\eta_{2,1}$.} 
	\label{fig:IA_Graph}
\end{figure*} 
\begin{align}
\label{eq:IA_condition1}
\nu_{\eta_{4,5}}[t]g_k[t]&=\beta_{\eta_{(k+1)\Mod{K},4}}[t]h_{k1}[t]
\end{align}
for Layer 1, 
\begin{align}
\label{eq:IA_condition2}
\hspace{-0.75em}\beta_{\eta_{(k+2)\Mod{K},4}}[t]h_{k1}[t]=\beta_{\eta_{(k+2)\Mod{K},2}}[t]h_{k1}[t]+\nu_{\eta_{(k+2)\Mod{K},2}}[t]g_{k}[t]=\nu_{\eta_{(k+1)\Mod{K},5}}[t]g_{k}[t]
\end{align}
for Layer 2, and 
\begin{align}
\label{eq:IA_condition3}
&\nu_{\eta_{(k+2)\Mod{K},5}}[t]g_{k}[t]=\beta_{\eta_{(k+2)\Mod{K},1}}[t]h_{k1}[t]+\nu_{\eta_{(k+2)\Mod{K},1}}[t]g_{k}[t]\nonumber\\
&=\beta_{\eta_{(k+1)\Mod{K},3}}[t]h_{k1}[t]+\nu_{\eta_{(k+1)\Mod{K},3}}[t]g_{k}[t]
\end{align}    
for Layer 3. Under the given ZF and IA conditions (cf.  \eqref{eq:ZF_conditions} and \eqref{eq:IA_condition1}--\eqref{eq:IA_condition3}), the precoders are functions of the channels $\mathbf{g}[t]$ and $\mathbf{H}[t]$. We fix the precoder for symbol $\eta_{4,5}$ to
\begin{equation}\label{eq:precoder_d5}
\nu_{\eta_{4,5}}[t]=j_{13}[t]j_{23}[t]j_{33}[t]g_1[t]g_2[t]g_3[t]h_{11}[t]h_{21}[t]h_{31}[t],
\end{equation} where
\begin{subequations}
	\begin{align}
	j_{13}[t]&=g_2[t]h_{31}[t]-g_{3}[t]h_{21}[t],\\
	j_{23}[t]&=g_3[t]h_{11}[t]-g_{1}[t]h_{31}[t],\\
	j_{33}[t]&=g_1[t]h_{21}[t]-g_{2}[t]h_{11}[t].
	\end{align}		
\end{subequations} The remaining precoders scalars depend on $\nu_{\eta_{4,5}}[t]$ and can be computed by using \eqref{eq:precoder_d5} in \eqref{eq:ZF_conditions} and  \eqref{eq:IA_condition1}--\eqref{eq:IA_condition3}. To this end, we compute the precoders along the $r$-th alignment chain, $r\in[K]=[3]$, of the graph (the first chain in Fig. \ref{fig:IA_Graph} for instance being the entire path from node $\eta_{4,5}$ to $\eta_{3,1}$) as a function of $\nu_{\eta_{4,5}}[t]$. The resulting precoders then become: \begin{subequations}
\label{eq:all_precoders_function_d5}
	\begin{align}
	\beta_{\eta_{r,4}}[t]&=\nu_{\eta_{4,5}}[t]\cdot\frac{g_{(r+2)\Mod{K}}[t]}{h_{(r+2)\Mod{K},1}[t]},\\\mathbf{p}_{\eta_{r,2}}[t]&\triangleq\begin{pmatrix}
	\nu_{\eta_{r,2}}[t] \\\beta_{\eta_{r,2}}[t]
	\end{pmatrix}\nonumber\\&=\nu_{\eta_{4,5}}[t]\cdot\frac{g_{(r+2)\Mod{K}}[t]h_{(r+1)\Mod{K},1}[t]}{j_{r,3}[t]}\begin{pmatrix}
	1 \\ -\frac{g_{(r+2)\Mod{K}}[t]}{h_{(r+2)\Mod{K},1}[t]}
	\end{pmatrix},\label{eq:concatenated_prec_1}\\
	\nu_{\eta_{(r+2)\Mod{K},5}}[t]&=\nu_{\eta_{4,5}}[t]\cdot\frac{g_{(r+2)\Mod{K}}[t]h_{(r+1)\Mod{K},1}[t]}{h_{(r+2)\Mod{K},1}[t]g_{(r+1)\Mod{K}}[t]}, \\\mathbf{p}_{\eta_{(r+1)\Mod{K},3}}[t]&\triangleq\begin{pmatrix}
	\nu_{\eta_{(r+1)\Mod{K},3}}[t] \\\beta_{\eta_{(r+1)\Mod{K},3}}[t]
	\end{pmatrix}\nonumber\\&=\nu_{\eta_{4,5}}[t]\cdot\frac{g_{(r+2)\Mod{K}}[t]h_{(r+1)\Mod{K},1}[t]g_r[t]}{g_{(r+1)\Mod{K}}[t]j_{(r+1)\Mod{K},3}[t]}\begin{pmatrix}
	-1 \\ \frac{g_{(r+2)\Mod{K}}[t]}{h_{(r+2)\Mod{K},1}[t]}
	\end{pmatrix},\label{eq:concatenated_prec_2}\\\mathbf{p}_{\eta_{(r+2)\Mod{K},1}}[t]&\triangleq\begin{pmatrix}
	\nu_{\eta_{(r+2)\Mod{K},1}}[t] \\\beta_{\eta_{(r+2)\Mod{K},1}}[t]
	\end{pmatrix}\nonumber\\&=\nu_{\eta_{4,5}}[t]\cdot\frac{g_{(r+2)\Mod{K}}[t]h_{(r+1)\Mod{K},1}[t]g_r[t]}{h_{(r+2)\Mod{K},1}[t]j_{(r+2)\Mod{K},3}[t]}\begin{pmatrix}
	\frac{h_{(r+1)\Mod{K},1}[t]}{g_{(r+1)\Mod{K}}[t]} \\ -1
	\end{pmatrix}\label{eq:concatenated_prec_3}.
	\end{align}		
\end{subequations} Taking a closer look at the \emph{concatenated} precoding vectors in \eqref{eq:concatenated_prec_1}, \eqref{eq:concatenated_prec_2} and \eqref{eq:concatenated_prec_3}, we see that these vectors are orthogonal to \begin{subequations}\label{eq:orthogonal_vectors}
\begin{align}
\mathbf{p}^{\perp}_{\eta_{(r+1)\Mod{K},3}}[t]=\mathbf{p}^{\perp}_{\eta_{r,2}}[t]=\mathbf{\tilde{h}}_{(r+2)\Mod{K}}[t]&\triangleq\begin{pmatrix}
g_{(r+2)\Mod{K}}[t] \\ h_{(r+2)\Mod{K},1}[t]
\end{pmatrix},\\\mathbf{p}^{\perp}_{\eta_{(r+2)\Mod{K},1}}[t]=\mathbf{\tilde{h}}_{(r+1)\Mod{K}}[t]&\triangleq\begin{pmatrix}
g_{(r+1)\Mod{K}}[t] \\ h_{(r+1)\Mod{K},1}[t]
\end{pmatrix}.
\end{align}
\end{subequations} This observation is in agreement with the ZF conditions \eqref{eq:ZF_conditions}. 

For reason of completeness, we would like to emphasize that our beamforming design also works with constant channels under the umbrella of \emph{real interference alignment} \cite{Motahari14,Maddah-Ali10}. Whether a two-phase precoding design with constant channels (similar to previous work on relay-aided X-channels \cite{Frank2014}) attains close-to-optimal performance is an interesting extension to work on. However, it is beyond the scope of this paper. Now we will go through the decoding from the perspective of both the RN and the UEs. 

\subsubsection*{Decoding at RN and the UEs}
To write both the received signal at UE$_k$, $k\in[K]$, and the RN, we introduce some additional notation. To this end, we define three \emph{distinct} subchain indices $\bar{r}_k,r'_k,\tilde{r}_k\in[K]$, that satisfy
\begin{equation}\label{eq:subchain_indices_def}
\bar{r}_k=(r'_k+1)\Mod{K}=(\tilde{r}_k+2)\Mod{K}=k,
\end{equation} $\forall k\in[K]$. 
%We concatenate these three indices in ascending order to generate the set $\mathcal{R}\triangleq[K]$, such that $\mathcal{R}[1]=\min\{\bar{r}_k,r'_k,\tilde{r}_k\}=1$ and $\mathcal{R}[3]=\min\{\bar{r}_k,r'_k,\tilde{r}_k\}=3$.
Exploiting %the definitions \eqref{eq:orthogonal_vectors} and 
the introduction of the subchain indices in \eqref{eq:subchain_indices_def}, 
we can write the received signal at the $k$-th UE as follows:
%\begin{align}
%\label{eq:rx_sig_k_th_UE_decoding}
%y_{u,k}[t]=\sum_{r\in\{\bar{r}_k,r'_k,\tilde{r}_k\}}\big(\mathbf{p}^{\perp}_{\eta_{r,2}}[t]\big)^{\dagger}
%\end{align} 
\begin{align}
\label{eq:rx_sig_k_th_UE_decoding}
y_{u,k}[t]=&\sum_{r\in\{\bar{r}_k,r'_k,\tilde{r}_k\}}\Bigg\{\mathbf{\tilde{h}}^{\dagger}_{(r_k'+1)\Mod{K}}[t]\mathbf{p}_{\eta_{(r+2)\Mod{K},1}}[t]\eta_{(r+2)\Mod{K},1}\nonumber\\&\quad\:\:+\mathbf{\tilde{h}}^{\dagger}_{(\tilde{r}_k+2)\Mod{K}}[t]\Big[\mathbf{p}_{\eta_{r,2}}[t]\eta_{r,2}+\mathbf{p}_{\eta_{(r+1)\Mod{K},3}}[t]\eta_{(r+1)\Mod{K},3}\Big]+h_{\bar{r}_k,1}[t]\beta_{\eta_{r,4}}[t]\eta_{r,4}\nonumber\\&\quad\:\:+g_{\bar{r}_k}[t]\nu_{\eta_{(r+2)\Mod{K},5}}[t]\eta_{(r+2)\Mod{K},5}\Bigg\}+g_k[t]\nu_{\eta_{4,5}}[t]\eta_{4,5}+z_{u,k}[t]\nonumber\\&\stackrel{(I)}=\mathbf{\tilde{h}}^{\dagger}_{(\tilde{r}_k+2)\Mod{K}}[t]\mathbf{p}_{\eta_{(\tilde{r}_k+2)\Mod{K},1}}[t]\eta_{(\tilde{r}_k+2)\Mod{K},1}+\mathbf{\tilde{h}}^{\dagger}_{\bar{r}_k}[t]\mathbf{p}_{\eta_{\bar{r}_k,2}}[t]\eta_{\bar{r}_k,2}\nonumber\\&\quad\:\:+\mathbf{\tilde{h}}^{\dagger}_{(r_k'+1)\Mod{K}}[t]\mathbf{p}_{\eta_{(r_k'+1)\Mod{K},3}}[t]\eta_{(r_k'+1)\Mod{K},3}+h_{\bar{r}_k,1}[t]\beta_{\eta_{\bar{r}_k,4}}[t]\eta_{\bar{r}_k,4}\nonumber\\&\quad\:\:+g_{(\tilde{r}_k+2)\Mod{K}}[t]\nu_{\eta_{(\tilde{r}_k+2)\Mod{K},5}}[t]\eta_{(\tilde{r}_k+2)\Mod{K},5}+g_{(\tilde{r}_k+2)\Mod{K}}[t]\nu_{\eta_{4,5}}[t]\eta_{4,5}\nonumber\\&\quad\:\:+h_{(\tilde{r}_k+2)\Mod{K},1}[t]\beta_{\eta_{\tilde{r}_k,4}}[t]\eta_{\tilde{r}_k,4}+h_{(r_k'+1)\Mod{K},1}[t]\beta_{\eta_{r_k',4}}[t]\eta_{r_k',4}\nonumber\\&\quad\:\:+\mathbf{\tilde{h}}^{\dagger}_{(r_k'+1)\Mod{K}}[t]\mathbf{p}_{\eta_{r_k',2}}[t]\eta_{r_k',2}+g_{(r_k'+1)\Mod{K}}[t]\nu_{\eta_{(r_k'+2)\Mod{K},5}}[t]\eta_{(r_k'+2)\Mod{K},5}\nonumber\\&\quad\:\:+g_{\bar{r}_k}[t]\nu_{\eta_{(\bar{r}_k+2)\Mod{K},5}}[t]\eta_{(\bar{r}_k+2)\Mod{K},5}+\mathbf{\tilde{h}}^{\dagger}_{\bar{r}_k}[t]\mathbf{p}_{\eta_{(\bar{r}_k+1)\Mod{K},3}}[t]\eta_{(\bar{r}_k+1)\Mod{K},3}\nonumber\\&\quad\:\:+\mathbf{\tilde{h}}^{\dagger}_{\bar{r}_k}[t]\mathbf{p}_{\eta_{(\bar{r}_k+2)\Mod{K},1}}[t]\eta_{(\bar{r}_k+2)\Mod{K},1}+z_{u,k}[t]
\end{align} In step $(I)$, we used the orthogonality conditions of \eqref{eq:orthogonal_vectors} as well as the definition \eqref{eq:subchain_indices_def}. Next, we insert Eq. \eqref{eq:all_precoders_function_d5} into \eqref{eq:rx_sig_k_th_UE_decoding} to rewrite $\frac{y_{u,k}[t]}{\nu_{\eta_{4,5}}[t]}$ according to:
\begin{align}\label{eq:rx_sig_UEk_M1_K3}
\frac{y_{u,k}[t]}{\nu_{\eta_{4,5}}[t]}=&-\frac{g_{(\tilde{r}_k+2)\Mod{K}}[t]h_{(\tilde{r}_k+1)\Mod{K},1}[t]j_{\tilde{r}_k,3}[t]g_{\tilde{r}_k}[t]}{h_{(\tilde{r}_k+2)\Mod{K},1}[t]g_{(\tilde{r}_k+1)\Mod{K}}[t]j_{(\tilde{r}_k+2)\Mod{K},3}[t]}\eta_{(\tilde{r}_k+2)\Mod{K},1}\nonumber\\&\quad\:\:-\frac{g_{(\bar{r}_k+2)\Mod{K}}[t]h_{(\bar{r}_k+1)\Mod{K},1}[t]j_{(\bar{r}_k+1)\Mod{K},3}[t]}{h_{(\bar{r}_k+2)\Mod{K},1}[t]j_{\bar{r}_k,3}[t]}\eta_{\bar{r}_k,2}\nonumber\\&\quad\:\:-\frac{g_{(r_k'+2)\Mod{K}}[t]h_{(r_k'+1)\Mod{K},1}[t]j_{r_k',3}[t]g_{r_k'}[t]}{h_{(r_k'+2)\Mod{K},1}[t]g_{(r_k'+1)\Mod{K}}[t]j_{(r_k'+1)\Mod{K},3}[t]}\eta_{(r_k'+1)\Mod{K},3}\nonumber\\&\quad\:\:+\frac{g_{(\bar{r}_k+2)\Mod{K}}[t]h_{\bar{r}_k,1}[t]}{h_{(\bar{r}_k+2)\Mod{K},1}[t]}\eta_{\bar{r}_k,4}+\frac{g^{2}_{(\tilde{r}_k+2)\Mod{K}}[t]h_{(\tilde{r}_k+1)\Mod{K},1}[t]}{h_{(\tilde{r}_k+2)\Mod{K},1}[t]g_{(\tilde{r}_k+1)\Mod{K}}[t]}\eta_{(\tilde{r}_k+2)\Mod{K},5}\nonumber\\&\quad\:\:+g_{(\tilde{r}_k+2)\Mod{K}}[t]\big(\eta_{\tilde{r}_k,4}+\eta_{4,5}\big)\nonumber\\&\quad\:\:+\frac{g_{(r_k'+2)\Mod{K}}[t]h_{(r_k'+1)\Mod{K},1}[t]}{h_{(r_k'+2)\Mod{K},1}[t]}\big(\eta_{r_k',4}+\eta_{r_k',2}+\eta_{(r_k'+2)\Mod{K},5}\big)\nonumber\\&\quad\:\:+\frac{g_{(\bar{r}_k+2)\Mod{K}}[t]h_{(\bar{r}_k+1)\Mod{K},1}[t]g_{\bar{r}_k}[t]}{h_{(\bar{r}_k+2)\Mod{K},1}[t]g_{(\bar{r}_k+1)\Mod{K}}[t]}\big(\eta_{(\bar{r}_k+2)\Mod{K},5}+\eta_{(\bar{r}_k+1)\Mod{K},3}\nonumber\\&\quad\:\:+\eta_{(\bar{r}_k+2)\Mod{K},1}\big)+\frac{z_{u,k}[t]}{\nu_{\eta_{4,5}}[t]}
\end{align} At the RN, on the other hand, the knowledge of $\eta_{i,j},i,j\in[3],$ as side information prefetched in its cache is exploited to cancel the contribution of these components. Thus, at the $t$-th channel use, the RN observes 
\begin{align}\label{eq:rx_sig_RN_M1_K3}
\frac{y_{r,1}'[t]}{\nu_{\eta_{4,5}}[t]}=&f_{1}[t]\sum_{i=1}^{4}\frac{\nu_{\eta_{i,5}}[t]}{\nu_{\eta_{4,5}}[t]}\eta_{i,5}+\frac{z_{r,1}[t]}{\nu_{\eta_{4,5}}[t]}\nonumber\\=&f_{1}[t]\Bigg(\eta_{4,5}+\frac{g_1[t]h_{31}[t]}{h_{11}[t]g_{3}[t]}\eta_{1,5}+\frac{g_2[t]h_{11}[t]}{h_{21}[t]g_{1}[t]}\eta_{2,5}+\frac{g_3[t]h_{21}[t]}{h_{31}[t]g_{2}[t]}\eta_{3,5}\Bigg)+\frac{z_{r,1}[t]}{\nu_{\eta_{4,5}}[t]}.
\end{align} Recall that the scheme spans over $T=8$ channel uses. Thus, due to the time-variant nature of the wireless channel, the UEs and the RN have 8 (noise-corrupted) linear \emph{independent} observations $\{y_{u,k}[t]\}_{t=1}^{8}$ and $\{y_{r,1}'[t]\}_{t=1}^{8}$ (in the field of reals $\mathbb{R}$) according to \eqref{eq:rx_sig_UEk_M1_K3} and \eqref{eq:rx_sig_RN_M1_K3}, respectively. In consequence, UE$_k$, $k\in[3]$, on the one hand, is able to decode its 5 \emph{desired} symbols 
\begin{itemize}
	\item $\eta_{(\tilde{r}_k+2)\Mod{K},1}$, $\eta_{\bar{r}_k,2}$, $\eta_{(r_k'+1)\Mod{K},3}$, $\eta_{\bar{r}_k,4}$, $\eta_{(\tilde{r}_k+2)\Mod{K},5}$
\end{itemize} and 3 \emph{aligned} interfering symbols
\begin{itemize}
	\item $\eta_{\tilde{r}_k,4}+\eta_{4,5}$,
	\item $\eta_{r_k',4}+\eta_{r_k',2}+\eta_{(r_k'+2)\Mod{K},5}$
	\item and $\eta_{(\bar{r}_k+2)\Mod{K},5}+\eta_{(\bar{r}_k+1)\Mod{K},3}+\eta_{(\bar{r}_k+2)\Mod{K},1}$,
\end{itemize} while the RN, on the other hand, decodes its desired symbol $\eta_{4,5}$ and 3 interfering (but not aligned) symbols $\eta_{1,5}$, $\eta_{2,5}$ and $\eta_{3,5}$. 
% This is due to the fact that, the time-variant nature of the channel allows both the RN and the UEs to receive $8$ (noise-corrupted) independent observations of its received signal components. 
In fact, as far as the RN is concerned, it actually only requires $4$ channel uses to allow for the decoding of the aforementioned symbols. The UEs are the reason why the scheme spans over $8$, and not $4$, channel uses. Consequently, the achievable NDT becomes $\frac{8}{5}$. Next, we present the NDT-optimal schemes for which $M=2$ and $K\leq 2$. 

\subsection{Achievability for $M=2$}\label{subsec:ach_M2}        

In the following, we will outline the delivery time optimal schemes for $M=2$ and $K\leq 2$. The following proposition states the achievable NDT.

\begin{proposition}\label{prop_M2}
	The achievable NDT of the network under study for $M=2$ RNs, $K=\{1,2\}$ UEs and $\mu\in[0,1]$ is given by 
	\begin{equation}
	\label{eq:ach_NDT_M_2_K_12}
	\delta(\mu)=\begin{cases}\max\Big\{1,3-4\mu\Big\}\quad&\text{ if } K= 1\\\max\bigg\{4-6\mu,\frac{4-3\mu}{2},\frac{3-\mu}{2}\bigg\}\quad&\text{ if }K=2\end{cases}.
	\end{equation}
\end{proposition}

\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.475\textwidth}
		\centering
		\begin{tikzpicture}[scale=0.8]
		\PlotNDTMTwoKOne
		\end{tikzpicture}
		\caption[NDT for $M=K=1$]{\small NDT for $M=2$ and $K=1$}
		\label{fig:NDT_M_K_2_1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.475\textwidth}  
		\centering 
		\begin{tikzpicture}[scale=0.8]
		\PlotNDTMTwoKTwo
		\end{tikzpicture}
		\caption[NDT for $M=1,K=2$]{\small NDT for $M=K=2$} 
		\label{fig:NDT_M_K_2_2}       
	\end{subfigure}
	\caption[NDT as a function of $\mu$ for $M=2$ and $K\leq 2$]
	{\small Optimal NDT as a function of $\mu$ for $M=2$ and $K\leq 2$} 
	\label{fig:NDT_M_K_2_LEQ_2}
\end{figure*} 

Now, we will present the proof of this proposition. Fig. \ref{fig:NDT_M_K_2_LEQ_2} shows that the achievable NDT in Proposition \ref{prop_M2} coincides with the lower bound. Due to Lemma \ref{corr_mu_0_and_1} and arguments of memory sharing, we will only establish the achievability of the corner point(s)
%\begin{itemize}
%	\item $\Big(\frac{1}{2},1\Big)$ 
%\end{itemize} 
$\Big(\frac{1}{2},1\Big)$
for $K=1$ and
%\begin{itemize}
%	\item $\Big(\frac{4}{9},\frac{4}{3}\Big)$, 
%	\item $\Big(\frac{1}{2},\frac{5}{4}\Big)$ 
%\end{itemize} 
$\Big(\frac{4}{9},\frac{4}{3}\Big)$, $\Big(\frac{1}{2},\frac{5}{4}\Big)$ for $K=2$, respectively. In this context, the NDT-optimal schemes for corner points $\Big(\frac{1}{2},1\Big)$ and $\Big(\frac{1}{2},\frac{5}{4}\Big)$ are based on the \emph{one-shot}\footnote{One-shot in this context is equivalent to requiring a \emph{single} channel use for conveying desired symbols to the receiving nodes.} reception of desired symbols, whereas at corner point $\Big(\frac{4}{9},\frac{4}{3}\Big)$ symbol decoding over multiple channel uses (similarly to the achievability for $M=1,K=3$ in subsection \ref{subsec:ach_M1}) is required. We start the achievability for the latter corner point $\Big(\frac{4}{9},\frac{4}{3}\Big)$.    

\subsubsection*{RNs Cache Placement}

\begin{figure}
	\FilesMTwoKThree
	\caption[Requested files by $K=2$ users and $M=2$ RNs]{\small Requested files by $K=2$ users and $M=2$ RNs and the availability illustrated by the symbols transmitted from the DeNB only or from both at the DeNB and one of the two RNs RN$_1$ and RN$_2$.}
	\label{fig:files_M_two_K_two}
\end{figure}

Again, we assume without loss of generality $N=4$ and that the UEs request files $W_1,W_2$ while RN$_1$ and RN$_2$ are interested in files $W_3$ and $W_4$, respectively. As shown in Fig. \ref{fig:files_M_two_K_two}, all files are comprised of $9$ symbols, i.e., the $i$-th file is composed of symbols $\eta_{i,1},\eta_{i,2},\ldots,\eta_{i,9}$. \emph{All} these symbols are available at the DeNB. In contrast, RN$_1$ and RN$_2$ prefetch symbols $\eta_{i,j},j=1,\ldots,4$ and $\eta_{i,l},l=5,\ldots,8$, respectively in its cache\footnote{We note that at $\mu=\nicefrac{4}{9}$, the joint cache content of the two RNs cannot contain the entire library of popular files.}. Since, RN$_1$ (RN$_2$) is, interested in file $W_3$ ($W_4$) and it knows a-priori $\eta_{3,j},j=1,\ldots,4$ ($\eta_{4,l},l=5,\ldots,8$), the missing symbols RN$_1$ (RN$_2$) desires are $\eta_{3,5},\eta_{3,6},\ldots,\eta_{3,9}$ ($\eta_{4,1},\ldots,\eta_{4,4}$ and $\eta_{4,9}$). In consequence, we design the transmission policy such that DeNB, RN$_1$ and RN$_2$ convey all receiving nodes with their desired symbols of files $W_1$ and $W_2$ as well as $\eta_{3,5},\eta_{3,6},\ldots,\eta_{3,9},\eta_{4,1},\ldots,\eta_{4,4}$ and $\eta_{4,9}$. These are in total $28$ information symbols. Next, we consider the encoding strategy for DeNB and RNs. 

\vspace{.5em}
\subsubsection*{Encoding at DeNB and RNs} 

\begin{figure}[h]
	\ZFMTwoKTwo
	\caption[Zero-forcing map]{\small Map that assigns which symbol to zero-force at which UE.} 
	\label{fig:ZF_Mtwo_Ktwo}
\end{figure} 

Similarly to the previously described scheme, we use the spatial correlation of shared symbols between RN$_1$ or RN$_2$ with the DeNB to facilitate ZF and IA at the UEs. However, leveraging all ZF opportunities at the UEs has one main drawback from the RNs perspective -- namely, it maximizes the number of interfering symbols imposed on RN$_1$ and RN$_2$. To limit this number, we do \emph{not} send symbols $\eta_{i,3},\eta_{i,4},\eta_{i,7}$ and $\eta_{i,8}$, $i=1,2$, through the DeNB (at the cost of missing these symbols' ZF opportunities) but rather through RN$_1$ or RN$_2$ directly to the UEs. (Effectively, this is as if the fractional cache size of the DeNB would be $\mu=\frac{5}{9}$.) All in all, this constitutes the transmit signals  
\begin{align}
\label{eq:tx_sig_DeNB_M2_K2}
x_s[t]&=\sum_{i_1=1}^{2}\sum_{\substack{j_1=1,\\j_1\neq \{3,4,7,8\}}}^{8}\nu_{\eta_{i_1,j_1}}[t]\eta_{i_1,j_1}+\sum_{j_2=5}^{8}\nu_{\eta_{3,j_2}}[t]\eta_{3,j_2}+\sum_{j_3=1}^{4}\nu_{\eta_{4,j_3}}[t]\eta_{4,j_3}+\sum_{i_2=1}^{4}\nu_{\eta_{i_2,9}}[t]\eta_{i_2,9},\\
\label{eq:tx_sig_RN1_M2_K2}
x_{r,m}[t]&=\sum_{\substack{i=1,\\i\neq m+2}}^{4}\sum_{j=4m-3}^{4m}\beta_{\eta_{i,j}}[t]\eta_{i,j},
\end{align} $\forall m\in[2]$ and $\forall t\in[T]$ for $T=12$, respectively. In above equation, the notation for the precoding scalars is identical to the one utilized in the previous achievability scheme. These scalars are, amongst others, chosen to fulfill the ZF conditions (cf. ZF map in Fig. \ref{fig:ZF_Mtwo_Ktwo}) for $j=1,2$ at UE$_k$: \begin{subequations}\label{eq:ZF_conditions_Mtwo_Ktwo}
	\begin{align}
	\nu_{\eta_{(k+1)\Mod{K},j}}[t]g_k[t]+\beta_{\eta_{(k+1)\Mod{K},j}}[t]h_{k1}[t]&=0,\label{eq:subseq_ZF_condition_1_M2K2}\\
	\nu_{\eta_{(k+1)\Mod{K},4+j}}[t]g_k[t]+\beta_{\eta_{(k+1)\Mod{K},4+j}}[t]h_{k2}[t]&=0,\label{eq:subseq_ZF_condition_2_M2K2}\\
	\nu_{\eta_{3,2(k+1)+j}}[t]g_k[t]+\beta_{\eta_{3,2(k+1)+j}}[t]h_{k2}[t]&=0,\\	\nu_{\eta_{4,2(k-1)+j}}[t]g_k[t]+\beta_{\eta_{4,2(k-1)+j}}[t]h_{k1}[t]&=0.
	\end{align}
\end{subequations} In addition to the ZF conditions, we also impose additional IA conditions to the precoding design (as shown in Fig. \ref{fig:IA_Graph_M2_K2}), which are for UE$_k$:
\begin{subequations}\label{eq:IA_conditions_Mtwo_Ktwo}
 	\begin{align}
	\nu_{\eta_{5-k,9}}[t]g_{k}[t]&=\beta_{\eta_{(k+1)\Mod{K},3}}[t]h_{k1}[t]=\beta_{\eta_{(k+1)\Mod{K},7}}[t]h_{k2}[t],\\
	\nu_{\eta_{k+2,9}}[t]g_{k}[t]&=\nu_{\eta_{4,6-2k}}[t]g_{k}[t]+\beta_{\eta_{4,6-2k}}[t]h_{k1}[t]=\beta_{\eta_{(k+1)\Mod{K},8}}[t]h_{k2}[t]\nonumber\\&=\nu_{\eta_{3,10-2k}}[t]g_{k}[t]+\beta_{\eta_{3,10-2k}}[t]h_{k2}[t],\\\nu_{\eta_{(k+1)\Mod{K},9}}[t]g_{k}[t]&=\nu_{\eta_{4,5-2k}}[t]g_{k}[t]+\beta_{\eta_{4,5-2k}}[t]h_{k1}[t]=\beta_{\eta_{(k+1)\Mod{K},4}}[t]h_{k1}[t]\nonumber\\&=\nu_{\eta_{3,9-2k}}[t]g_{k}[t]+\beta_{\eta_{3,9-2k}}[t]h_{k2}[t].
 	\end{align}
 \end{subequations} As opposed to all other symbols in \eqref{eq:IA_conditions_Mtwo_Ktwo}, symbols $\eta_{(k+1)\Mod{K},j}$ and $\eta_{(k+1)\Mod{K},4+j}$, $j=1,2$ (in total 8), are only subjected to ZF conditions \eqref{eq:subseq_ZF_condition_1_M2K2} and \eqref{eq:subseq_ZF_condition_2_M2K2} but not to any alignment conditions. This is due to the fact these are ZF symbols that are canceled at one of the UEs while being desired at the other UE. In consequence, we do not need to align these symbols at any UE. However, as $\eta_{(k+1)\Mod{K},1}$ and $\eta_{(k+1)\Mod{K},2}$ have \emph{identical} ZF conditions (similarly for the pair of symbols $\eta_{(k+1)\Mod{K},5}, \eta_{(k+1)\Mod{K},6}$), we need to distinguish these symbols at UE$_k$ for the sake of reliable decodability. To this end, we introduce additional complex random factors $c_{\eta_{(k+1)\Mod{K},j}}[t]$ and $c_{\eta_{(k+1)\Mod{K},4+j}}[t]$, $j=1,2$, when fixing the precoding scalars $\nu_{\eta_{(k+1)\Mod{K},j}}[t],\beta_{\eta_{(k+1)\Mod{K},j}}[t]$
 and $\nu_{\eta_{(k+1)\Mod{K},4+j}}[t],\beta_{\eta_{(k+1)\Mod{K},4+j}}[t]$. These random factors are \emph{a-priori} known by all transmitting and receiving nodes.  
 \begin{figure*}[h]
 	\centering
 	\begin{tikzpicture}[scale=1]
 	\AlignGraphMTwoKTwo
 	\end{tikzpicture}
 	\caption[Interference Alignment Graph for the achievability at corner point $(\frac{4}{9},\frac{4}{3})$ for $M=2$ and $K=2$]{\small Interference Alignment Graph from the UE perspective for the achievability at corner point $(\frac{4}{9},\frac{4}{3})$ for $M=2$ and $K=2$. The graph consists of six alignment chains and 20 nodes (i.e., symbols). The remaining 8 symbols ($\eta_{(k+1)\Mod{K},j}$, $\eta_{(k+1)\Mod{K},4+j}$, $j,k=1,2$) do not appear in the alignment graph as these symbols are zero-forced at the unwanted UE (according to the ZF conditions \eqref{eq:subseq_ZF_condition_1_M2K2} and \eqref{eq:subseq_ZF_condition_2_M2K2}) while they are desired by the other UE.} 
 	\label{fig:IA_Graph_M2_K2}
 \end{figure*} 
 
 Now we provide the solution of the system of equations comprising of ZF and IA conditions. For this purpose, we determine the precoding scalars in all 6 alignment chains as a function of $\nu_{\eta_{1,9}}[t],\nu_{\eta_{2,9}}[t],\nu_{\eta_{3,9}}[t]$ or $\nu_{\eta_{4,9}}[t]$. Hereby, we fix these scalars to
% \begin{subequations}
% 	\begin{align}
% 	\nu_{\eta_{1,9}}[t]&=l_{13}[t]l_{23}[t]h_{21}[t],\\
% 	\nu_{\eta_{2,9}}[t]&=l_{13}[t]l_{23}[t]h_{11}[t],\\
% 	\nu_{\eta_{3,9}}[t]&=l_{13}[t]l_{23}[t]h_{12}[t]h_{21}[t]h_{22}[t],\\
% 	\nu_{\eta_{4,9}}[t]&=l_{13}[t]l_{23}[t]h_{11}[t]h_{12}[t]h_{21}[t].
% 	\end{align}
%\end{subequations}
 \begin{subequations}
 	\begin{align}\label{eq:prec_nu_eta_i9}
 	\nu_{\eta_{(k+1)\Mod{K},9}}[t]&=l_{13}[t]l_{23}[t]h_{k1}[t],\\
 	\nu_{\eta_{5-k,9}}[t]=\nu_{\eta_{(k+1)\Mod{K}+2,9}}[t]&=l_{13}[t]l_{23}[t]h_{k1}[t]h_{k2}[t]h_{(k+1)\Mod{K},2}[t],
 	\end{align}
 \end{subequations} where
 \begin{subequations}\label{eq:l13_l23_def}
 	\begin{align}
 	l_{13}[t]&=g_{1}[t]h_{21}[t]-g_{2}[t]h_{11}[t],\\
 	l_{23}[t]&=g_{2}[t]h_{12}[t]-g_{1}[t]h_{22}[t].
 	\end{align}
 \end{subequations} As a consequence, the precoders become:
 \begin{subequations}\label{eq:all_precoders_function_M2_K2}
 	\begin{align}
 	\mathbf{p}_{\eta_{(k+1)\Mod{K},j}}[t]&\triangleq\begin{pmatrix}
 	\nu_{\eta_{(k+1)\Mod{K},j}}[t] \\ \beta_{\eta_{(k+1)\Mod{K},j}}[t]
 	\end{pmatrix}=c_{\eta_{(k+1)\Mod{K},j}}[t]\begin{pmatrix}
 	h_{k1}[t] \\ -g_{k}[t]
 	\end{pmatrix},  \label{eq:concat_bf_1}  \\
 	\beta_{\eta_{(k+1)\Mod{K},3}}[t]&=\nu_{\eta_{(k+1)\Mod{K}+2,9}}[t]\frac{g_k[t]}{h_{k1}[t]}, \\ 	
    \beta_{\eta_{(k+1)\Mod{K},4}}[t]&=\nu_{\eta_{(k+1)\Mod{K},9}}[t]\frac{g_k[t]}{h_{k1}[t]},\\
 	\mathbf{p}_{\eta_{(k+1)\Mod{K},4+j}}[t]&\triangleq\begin{pmatrix}
 	\nu_{\eta_{(k+1)\Mod{K},4+j}}[t] \\ \beta_{\eta_{(k+1)\Mod{K},4+j}}[t]
 	\end{pmatrix}=c_{\eta_{(k+1)\Mod{K},4+j}}[t]\begin{pmatrix}
 	-h_{k2}[t] \\ g_{k}[t]
 	\end{pmatrix}, \label{eq:concat_bf_2}\\
    \beta_{\eta_{(k+1)\Mod{K},7}}[t]&=\nu_{\eta_{(k+1)\Mod{K}+2,9}}[t]\frac{g_k[t]}{h_{k2}[t]}, \\
 	\beta_{\eta_{(k+1)\Mod{K},8}}[t]&=\nu_{\eta_{k+2,9}}[t]\frac{g_k[t]}{h_{k2}[t]}, \\
 	\mathbf{p}_{\eta_{3,9-2k}}[t]&\triangleq\begin{pmatrix}
 	\nu_{\eta_{3,9-2k}}[t] \\ \beta_{\eta_{3,9-2k}}[t]
 	\end{pmatrix}=(-1)^{k+1}\nu_{\eta_{(k+1)\Mod{K},9}}[t]\frac{g_k[t]}{l_{23}[t]}\begin{pmatrix}
 	-h_{(k+1)\Mod{K},2}[t] \\ g_{(k+1)\Mod{K}}[t]
 	\end{pmatrix}, \label{eq:concat_bf_3}\\
 	\mathbf{p}_{\eta_{3,10-2k}}[t]&\triangleq\begin{pmatrix}
 	\nu_{\eta_{3,10-2k}}[t] \\ \beta_{\eta_{3,10-2k}}[t]
 	\end{pmatrix}=(-1)^{k+1}\nu_{\eta_{k+2,9}}[t]\frac{g_k[t]}{l_{23}[t]}\begin{pmatrix}
 	-h_{(k+1)\Mod{K},2}[t] \\ g_{(k+1)\Mod{K}}[t]
 	\end{pmatrix},	\label{eq:concat_bf_4}\\
 	\mathbf{p}_{\eta_{4,5-2k}}[t]&\triangleq\begin{pmatrix}
 	\nu_{\eta_{4,5-2k}}[t] \\ \beta_{\eta_{4,5-2k}}[t]
 	\end{pmatrix}=(-1)^{k+1}\nu_{\eta_{(k+1)\Mod{K},9}}[t]\frac{g_k[t]}{l_{13}[t]}\begin{pmatrix}
 	h_{(k+1)\Mod{K},1}[t] \\ -g_{(k+1)\Mod{K}}[t]
 	\end{pmatrix}, \label{eq:concat_bf_5}\\
 	\mathbf{p}_{\eta_{4,6-2k}}[t]&\triangleq\begin{pmatrix}
 	\nu_{\eta_{4,6-2k}}[t] \\ \beta_{\eta_{4,6-2k}}[t]
 	\end{pmatrix}=(-1)^{k+1}\nu_{\eta_{k+2,9}}[t]\frac{g_k[t]}{l_{13}[t]}\begin{pmatrix}
 	h_{(k+1)\Mod{K},1}[t] \\ -g_{(k+1)\Mod{K}}[t]
 	\end{pmatrix} \label{eq:concat_bf_6}.
 	\end{align}
 \end{subequations} Hereby, the concatenated beamforming vectors in \eqref{eq:concat_bf_1},\eqref{eq:concat_bf_2} and \eqref{eq:concat_bf_3}--\eqref{eq:concat_bf_6} are perpendicular to \begin{subequations}\label{eq:perp_vectors}
  	\begin{align}
	\mathbf{p}^{\perp}_{\eta_{(k+1)\Mod{K},j}}[t]=\mathbf{\tilde{h}}_{k1}[t]&\triangleq\begin{pmatrix}
  	g_{k}[t] \\ h_{k1}[t]
  	\end{pmatrix},\\	\mathbf{p}^{\perp}_{\eta_{(k+1)\Mod{K},4+j}}[t]=\mathbf{\tilde{h}}_{k2}[t]&\triangleq\begin{pmatrix}
  	g_{k}[t] \\ h_{k2}[t]
  	\end{pmatrix},\\
  	\mathbf{p}^{\perp}_{\eta_{3,10-2k}}[t]=\mathbf{p}^{\perp}_{\eta_{3,9-2k}}[t]=\mathbf{\tilde{h}}_{(k+1)\Mod{K},2}[t]&\triangleq\begin{pmatrix}
  	g_{(k+1)\Mod{K}}[t] \\ h_{(k+1)\Mod{K},2}[t]
  	\end{pmatrix}, \\
  	\mathbf{p}^{\perp}_{\eta_{4,6-2k}}[t]=\mathbf{p}^{\perp}_{\eta_{4,5-2k}}[t]=\mathbf{\tilde{h}}_{(k+1)\Mod{K},1}[t]&\triangleq\begin{pmatrix}
  	g_{(k+1)\Mod{K}}[t] \\ h_{(k+1)\Mod{K},1}[t]
  	\end{pmatrix}.
  	\end{align}
  \end{subequations} This observation concurs with the four ZF conditions of Eq. \eqref{eq:ZF_conditions_Mtwo_Ktwo}. The decoding at RNs and UEs is described next. 
   
\subsubsection*{Decoding at the RNs and the UEs} In the following, we will formulate the received signals of the RNs and the UEs. In the equations to come, we will use the index $k'$ which satisfies
\begin{equation}
(k'+1)\Mod{K}=k
\end{equation} for $k\in[K]$ to write $y_{u,k}[t]$ in a compact form. Utilizing this definition and the orthogonality observations, $y_{u,k}[t]$ becomes:   
\begin{align}\label{eq:UE_rx_sig_M2_K2}
y_{u,k}[t]&=\sum_{s_1=1}^{2}\sum_{j=1}^{2}\bigg(\tilde{\mathbf{h}}^{\dagger}_{k1}[t]\mathbf{p}_{\eta_{(s_1+1)\Mod{K},j}}[t]\eta_{(s_1+1)\Mod{K},j}+\tilde{\mathbf{h}}^{\dagger}_{k2}[t]\mathbf{p}_{\eta_{(s_1+1)\Mod{K},4+j}}[t]\eta_{(s_1+1)\Mod{K},4+j}\bigg)\nonumber\\&\quad\:\:+h_{k1}[t]\sum_{s_2=1}^{2}\Big(\beta_{\eta_{(s_2+1)\Mod{K},3}}[t]\eta_{(s_2+1)\Mod{K},3}+\beta_{\eta_{(s_2+1)\Mod{K},4}}[t]\eta_{(s_2+1)\Mod{K},4}\Big)\nonumber\\&\quad\:\:+h_{k2}[t]\sum_{s_3=1}^{2}\Big(\beta_{\eta_{(s_3+1)\Mod{K},3}}[t]\eta_{(s_3+1)\Mod{K},3}+\beta_{\eta_{(s_3+1)\Mod{K},4}}[t]\eta_{(s_3+1)\Mod{K},4}\Big)\nonumber\\&\quad\:\:+\tilde{\mathbf{h}}^{\dagger}_{k1}[t]\sum_{s_4=1}^{2}\bigg(\mathbf{p}_{\eta_{4,5-2s_4}}[t]\eta_{4,5-2s_4}+\mathbf{p}_{\eta_{4,6-2s_4}}[t]\eta_{4,6-2s_4}\bigg)+\tilde{\mathbf{h}}^{\dagger}_{k2}[t]\sum_{s_5=1}^{2}\bigg(\mathbf{p}_{\eta_{3,9-2s_5}}[t]\eta_{3,9-2s_5}\nonumber\\&\quad\:\:+\mathbf{p}_{\eta_{3,10-2s_5}}[t]\eta_{3,10-2s_5}\bigg)+g_{k}[t]\sum_{s_6=1}^{2}\Big(\nu_{\eta_{(s_6+1)\Mod{K},9}}[t]\eta_{(s_6+1)\Mod{K},9}+\nu_{\eta_{s_6+2,9}}[t]\eta_{s_6+2,9}\Big)\nonumber\\&\quad\:\:+z_{u,k}[t]\nonumber\\&\stackrel{(II)}{=}\sum_{j=1}^{2}\bigg(\tilde{\mathbf{h}}^{\dagger}_{k1}[t]\mathbf{p}_{\eta_{(k'+1)\Mod{K},j}}[t]\eta_{(k'+1)\Mod{K},j}+\tilde{\mathbf{h}}^{\dagger}_{k2}[t]\mathbf{p}_{\eta_{(k'+1)\Mod{K},4+j}}[t]\eta_{(k'+1)\Mod{K},4+j}\bigg)\nonumber\\&\quad\:\:+h_{k1}[t]\Big(\beta_{\eta_{(k'+1)\Mod{K},3}}[t]\eta_{(k'+1)\Mod{K},3}+\beta_{\eta_{(k'+1)\Mod{K},4}}[t]\eta_{(k'+1)\Mod{K},4}\Big)\nonumber\\&\quad\:\:+h_{k2}[t]\Big(\beta_{\eta_{(k'+1)\Mod{K},7}}[t]\eta_{(k'+1)\Mod{K},7}+\beta_{\eta_{(k'+1)\Mod{K},8}}[t]\eta_{(k'+1)\Mod{K},8}\Big)\nonumber\\&\quad\:\:+g_{k}[t]\nu_{\eta_{(k'+1)\Mod{K},9}}[t]\eta_{(k'+1)\Mod{K},9}+\tilde{\mathbf{h}}^{\dagger}_{k1}[t]\Big(\mathbf{p}_{\eta_{4,5-2k}}[t]\eta_{4,5-2k}+\mathbf{p}_{\eta_{4,6-2k}}[t]\eta_{4,6-2k}\Big)\nonumber\\&\quad\:\:+\tilde{\mathbf{h}}^{\dagger}_{k2}[t]\Big(\mathbf{p}_{\eta_{3,9-2k}}[t]\eta_{3,9-2k}+\mathbf{p}_{\eta_{3,10-2k}}[t]\eta_{3,10-2k}\Big)+h_{k1}[t]\Big(\beta_{\eta_{(k+1)\Mod{K},3}}[t]\eta_{(k+1)\Mod{K},3}\nonumber\\&\quad\:\:+\beta_{\eta_{(k+1)\Mod{K},4}}[t]\eta_{(k+1)\Mod{K},4}\Big)+h_{k2}[t]\Big(\beta_{\eta_{(k+1)\Mod{K},7}}[t]\eta_{(k+1)\Mod{K},7}\nonumber\\&\quad\:\:+\beta_{\eta_{(k+1)\Mod{K},8}}[t]\eta_{(k+1)\Mod{K},8}\Big)+g_{k}[t]\Big(\nu_{\eta_{(k+1)\Mod{K},9}}[t]\eta_{(k+1)\Mod{K},9}\nonumber\\&\quad\:\:+\nu_{\eta_{(k'+1)\Mod{K}+2,9}}[t]\eta_{(k'+1)\Mod{K}+2,9}+\nu_{\eta_{(k+1)\Mod{K}+2,9}}[t]\eta_{(k+1)\Mod{K}+2,9}\Big)+z_{u,k}[t]
\end{align} Similarly to step $(I)$, step $(II)$ exploits the orthogonality conditions of \eqref{eq:perp_vectors} as well as the definition of index $k'$. The substition of Eq. \eqref{eq:all_precoders_function_M2_K2} into Eq. \eqref{eq:UE_rx_sig_M2_K2} then yields:     
\begin{align}\label{eq:rx_sig_UEk_M2_K2}
y_{u,k}[t]&=\sum_{j=1}^{2}\bigg((-1)^{k+1}c_{\eta_{(k'+1)\Mod{K},j}}[t]l_{13}[t]\eta_{(k'+1)\Mod{K},j}\nonumber\\&\quad\:\:+(-1)^{k+1}c_{\eta_{(k'+1)\Mod{K},4+j}}[t]l_{23}[t]\eta_{(k'+1)\Mod{K},4+j}\bigg)\nonumber\\&\quad\:\:+\frac{h_{k1}[t]g_{k'}[t]}{h_{k'1}[t]}\nu_{\eta_{(k'+1)\Mod{K}+2,9}}[t]\eta_{(k'+1)\Mod{K},3}+\frac{h_{k1}[t]g_{k'}[t]}{h_{k'1}[t]}\nu_{\eta_{(k'+1)\Mod{K},9}}[t]\eta_{(k'+1)\Mod{K},4}\nonumber\\&\quad\:\:+\frac{h_{k2}[t]g_{k'}[t]}{h_{k'2}[t]}\nu_{\eta_{(k'+1)\Mod{K}+2,9}}[t]\eta_{(k'+1)\Mod{K},7}+\frac{h_{k2}[t]g_{k'}[t]}{h_{k'2}[t]}\nu_{\eta_{(k+1)\Mod{K}+2,9}}[t]\eta_{(k'+1)\Mod{K},8}\nonumber\\&\quad\:\:+g_{k}[t]\nu_{\eta_{(k'+1)\Mod{K},9}}[t]\eta_{(k'+1)\Mod{K},9}+g_{k}[t]\nu_{\eta_{(k+1)\Mod{K},9}}[t]\big(\eta_{(k+1)\Mod{K},9}+\eta_{4,5-2k}\nonumber\\&\quad\:\:+\eta_{(k+1)\Mod{K},4}+\eta_{3,9-2k}\big)+g_{k}[t]\nu_{\eta_{(k+1)\Mod{K}+2,9}}[t]\big(\eta_{(k+1)\Mod{K}+2,9}+\eta_{(k+1)\Mod{K},3}\nonumber\\&\quad\:\:+\eta_{(k+1)\Mod{K},7}\big)+g_{k}[t]\nu_{\eta_{k+2,9}}[t]\big(\eta_{k+2,9}+\eta_{4,6-2k}+\eta_{(k+1)\Mod{K},8}+\eta_{3,10-2k}\big)+z_{u,k}[t]
\end{align} On the other hand, the received signals of RN$_1$ and RN$_2$ after canceling known interfering components (by exploiting the cache content) can be written as follows:
\begin{align}\label{eq:rx_sig_RN1_M2_K2}
y_{r,1}'[t]&=f_{1}[t]\bigg(\sum_{i_1=1}^{2}\sum_{j_1=5}^{6}\nu_{\eta_{i_1,j_1}}[t]\eta_{i_1,j_1}+\sum_{j_2=5}^{8}\nu_{\eta_{3,j_2}}[t]\eta_{3,j_2}+\sum_{i_2=1}^{4}\nu_{\eta_{i_2,9}}[t]\eta_{i_2,9}\bigg)+z_{r,1}[t]\nonumber\\&=f_{1}[t]\bigg(\nu_{\eta_{1,9}}[t]\frac{g_2[t]h_{12}[t]}{l_{23}[t]}\eta_{3,5}+\nu_{\eta_{4,9}}[t]\frac{g_2[t]h_{12}[t]}{l_{23}[t]}\eta_{3,6}-\nu_{\eta_{2,9}}[t]\frac{g_1[t]h_{22}[t]}{l_{23}[t]}\eta_{3,7}\nonumber\\&\quad\:\:-\nu_{\eta_{3,9}}[t]\frac{g_1[t]h_{22}[t]}{l_{23}[t]}\eta_{3,8}+\nu_{\eta_{3,9}}[t]\eta_{3,9}-c_{\eta_{1,5}}[t]h_{22}[t]\eta_{1,5}-c_{\eta_{1,6}}[t]h_{22}[t]\eta_{1,6}\nonumber\\&\quad\:\:-c_{\eta_{2,5}}[t]h_{12}[t]\eta_{2,5}-c_{\eta_{2,6}}[t]h_{12}[t]\eta_{2,6}+\nu_{\eta_{1,9}}[t]\eta_{1,9}+\nu_{\eta_{2,9}}[t]\eta_{2,9}\nonumber\\&\quad\:\:+\nu_{\eta_{4,9}}[t]\eta_{4,9}\bigg)+z_{r,1}[t],
\end{align} \begin{align}\label{eq:rx_sig_RN2_M2_K2}
y_{r,2}'[t]&=f_{2}[t]\bigg(\sum_{i_1=1}^{2}\sum_{j_1=1}^{2}\nu_{\eta_{i_1,j_1}}[t]\eta_{i_1,j_1}+\sum_{j_2=1}^{4}\nu_{\eta_{4,j_2}}[t]\eta_{4,j_2}+\sum_{i_2=1}^{4}\nu_{\eta_{i_2,9}}[t]\eta_{i_2,9}\bigg)+z_{r,2}[t]\nonumber\\&=f_{2}[t]\bigg(-\nu_{\eta_{1,9}}[t]\frac{g_2[t]h_{11}[t]}{l_{13}[t]}\eta_{4,1}-\nu_{\eta_{4,9}}[t]\frac{g_2[t]h_{11}[t]}{l_{13}[t]}\eta_{4,2}+\nu_{\eta_{2,9}}[t]\frac{g_1[t]h_{21}[t]}{l_{13}[t]}\eta_{4,3}\nonumber\\&\quad\:\:+\nu_{\eta_{3,9}}[t]\frac{g_1[t]h_{21}[t]}{l_{13}[t]}\eta_{4,4}+\nu_{\eta_{4,9}}[t]\eta_{4,9}+c_{\eta_{1,1}}[t]h_{21}[t]\eta_{1,1}+c_{\eta_{1,2}}[t]h_{21}[t]\eta_{1,2}\nonumber\\&\quad\:\:+c_{\eta_{2,1}}[t]h_{11}[t]\eta_{2,1}+c_{\eta_{2,2}}[t]h_{11}[t]\eta_{2,2}+\nu_{\eta_{1,9}}[t]\eta_{1,9}+\nu_{\eta_{2,9}}[t]\eta_{2,9}\nonumber\\&\quad\:\:+\nu_{\eta_{3,9}}[t]\eta_{3,9}\bigg)+z_{r,2}[t].
\end{align} When choosing the precoding scalars $\nu_{\eta_{i,9}}[t],i=1,\ldots,4$ independently (e.g., as in Eq. \eqref{eq:prec_nu_eta_i9}) in Eqs. \eqref{eq:rx_sig_UEk_M2_K2}--\eqref{eq:rx_sig_RN2_M2_K2} over $T=12$ channel uses for a time-varying wireless channel, both the RNs and the UEs make in total $12$ noise-corrupted independent observations $\{y_{u,k}[t]\}_{t=1}^{12}$ and $\{y_{r,m}'[t]\}_{t=1}^{12}$ as a function of their desired symbols and (possibly aligned) interfering symbols. This facilitates that UE$_k$, $k\in[2]$, on the one hand, is capable of decoding its $9$ desired symbols 
\begin{itemize}
	\item $\eta_{(k'+1)\Mod{K},j},j=1,2,\ldots,9$
\end{itemize} and $3$ distinct sums of interfering symbols in the form 
\begin{itemize}
	\item $\eta_{(k+1)\Mod{K},9}+\eta_{4,5-2k}+\eta_{(k+1)\Mod{K},4}+\eta_{3,9-2k}$,
	\item $\eta_{(k+1)\Mod{K}+2,9}+\eta_{(k+1)\Mod{K},3}+\eta_{(k+1)\Mod{K},7}$,
	\item and  $\eta_{k+2,9}+\eta_{4,6-2k}+\eta_{(k+1)\Mod{K},8}+\eta_{3,10-2k}$. 
\end{itemize} RN$_m$, $m\in[2]$, on the other hand, decodes its $5$ remaining uncached desired symbols ($\eta_{m+2,9-4m}$, $\eta_{m+2,10-4m}$, $\eta_{m+2,11-4m}$, $\eta_{m+2,12-4m}$ and $\eta_{m+2,9}$) and $7$ interfering symbols ($\eta_{1,9-4m}$, $\eta_{1,10-4m}$, $\eta_{2,9-4m}$, $\eta_{1,10-4m}$, $\eta_{1,9}$, $\eta_{2,9}$ and $\eta_{(m+1)\Mod{M}+2,9}$). As opposed to the previous scheme, both RNs and UEs require $T=12$ channel uses to determine their desired symbols. Since every file consists of $9$ symbols, the achievable NDT thus corresponds to $\frac{12}{9}=\frac{4}{3}$.

Now, we establish the achievability for corner points $\Big(\frac{1}{2},1\Big)$ (when $M=2,K=1$ as shown in Fig. \ref{fig:one_shot_M2_K1}) and $\Big(\frac{1}{2},\frac{5}{4}\Big)$ (when $M=2,K=2$ as shown in Fig. \ref{fig:one_shot_M2_K2}), respectively. These schemes are one-shot schemes that combine the Maddah-Ali Niesen (MAN) scheme with cooperative zero-forcing beamforming among DeNB and RNs. The generalized scheme is outlined in detail in Section \ref{cha_one_shot}. Thus, in the following, we will only briefly outline the achievability of these two corner points. We start with the cache placement at the RNs.

\subsubsection*{RNs cache placement}

At corner points $\Big(\frac{1}{2},1\Big)$ and $\Big(\frac{1}{2},\frac{5}{4}\Big)$, we assume that each file $W_i$ comprises of $L_1=2$ and $L_2=4$ symbols, respectively. Hereby, RN$_m$, $m=1,2,$ caches the $m$-th block of $\frac{L_1}{2}$ $\Big(\frac{L_2}{2}\Big)$ symbols. For instance, at corner point $\Big(\frac{1}{2},\frac{5}{4}\Big)$, RN$_2$ prefetches the last $\frac{L_2}{2}=2$ symbols ($\eta_{i,3}$ and $\eta_{i,4}$) of each file $W_i$ (cf. $S_2$ in Fig. \ref{fig:one_shot_M2_K2}).      

\begin{figure}[h]
	\begin{center}
		\AchMTwoKone
		\caption{\small One-shot scheme at corner point $\Big(\frac{1}{2},1\Big)$ for $M=2$ RNs, $K=1$ UEs and $N=3$ files. Each file $W_i,i=1,2,3,$ is comprised of two symbols $\eta_{i,1}$ and $\eta_{i,2}$. The figure shows, respectively, the DeNB transmit signal $x_s[t]$, the $m$-th RNs transmit signal $x_{r,m}[t]$, the received signals of UE$_1$ $y_{u,1}[t]$ and RN$_m$ $y_{r,m}'[t]$ (when RN$_m$ exploits its cached content $S_m$ as side information) that leads to an NDT of $1$ after $T=2$ channel uses.}	
		\label{fig:one_shot_M2_K1}
	\end{center}
\end{figure} 

\begin{figure}[h]
	\begin{center}
		\AchMTwoKTwo
		\caption{\small One-shot scheme at corner point $\Big(\frac{1}{2},\frac{5}{4}\Big)$ for $M=2$ RNs, $K=2$ UEs and $N=4$ files. Each file $W_i,i=1,2,3,$ is comprised of four symbols $\eta_{i,1},\eta_{i,2},\eta_{i,3}$ and $\eta_{i,4}$. The figure shows, respectively, the DeNB transmit signal $x_s[t]$, the $m$-th RNs transmit signal $x_{r,m}[t]$, the received signals of UE$_k$ $y_{u,k}[t]$ and RN$_m$ $y_{r,m}'[t]$ (when RN$_m$ exploits its cached content $S_m$ as side information) that leads to an NDT of $\frac{5}{4}$ after $T=5$ channel uses. We use $I(a_1,a_2,a_3)$ to denote a linear interference term as a function of the three symbols $a_1$, $a_2$ and $a_3$. Further, $l_{13}[t]$ and $l_{23}[t]$ are defined in Eq. \eqref{eq:l13_l23_def}.}	
		\label{fig:one_shot_M2_K2}
	\end{center}
\end{figure} 

\subsubsection*{Encoding at DeNB and RNs}

For both corner points, we use the first $T_1$\footnote{In the schemes of corner points $\Big(\frac{1}{2},1\Big)$ and $\Big(\frac{1}{2},\frac{5}{4}\Big)$, $T_1$ corresponds to $1$ and $2$ channel uses, respectively.} channel uses to multicast all symbols desired by RN$_1$ and RN$_2$ over the DeNB-RN broadcast channel. Simultaneously, we exploit the side information at the RNs caches to zero-force undesired symbols at one of the UEs and provide this particular UE with one of its desired symbols. For example, at $t=1$ for corner point $\Big(\frac{1}{2},\frac{5}{4}\Big)$, we multicast the symbols $\eta_{3,3}$ and $\eta_{4,1}$ at the DeNB in an MAN scheme manner according to:
\begin{equation}
x_{s}[1]=\nu_{\eta_{3,3}}[1]\eta_{3,3}+\nu_{\eta_{4,1}}[1]\eta_{4,1}
\end{equation} This transmit signal allows each RN to retrieve its desired symbol by exploiting its knowledge of the channel and of the undesired symbol in $x_{s}[1]$ through its cache (e.g., RN$_1$ is interested in symbol $\eta_{3,3}$ and has $\eta_{4,1}$ stored in its cache). However, neither UE$_1$ nor UE$_2$ are interested in the symbols of $x_s[1]$ ($\eta_{3,3},\eta_{4,1}$). Thus we do not only leverage the knowledge of RN$_1$ in $\eta_{4,1}$ and of RN$_2$ in $\eta_{3,3}$ from a receiver-caching perspective, but instead we also capitalize on this cognizance from a transmitter-caching perspective by sending
\begin{subequations}
	\begin{align}
	x_{r,1}[1]&=\beta_{\eta_{4,1}}[1]\eta_{4,1}+\eta_{1,1}\\
	x_{r,2}[1]&=\beta_{\eta_{3,3}}[1]\eta_{3,3}
	\end{align}
\end{subequations} from RN$_1$ and RN$_2$, respectively, to overcome this issue. Hereby, we choose the following concatenated vectors to satisfy:
\begin{subequations}
	\begin{align}
	\begin{pmatrix}
	\nu_{\eta_{3,3}}[1] \\ \beta_{\eta_{3,3}}[1]
	\end{pmatrix}&\perp \begin{pmatrix} g_1[1] \\ h_{12}[1]
	\end{pmatrix},\\ \begin{pmatrix}
	\nu_{\eta_{4,1}}[1] \\ \beta_{\eta_{4,1}}[1]
	\end{pmatrix}&\perp \begin{pmatrix} g_1[1] \\ h_{11}[1]
	\end{pmatrix}.
	\end{align}
\end{subequations} This facilitates that UE$_1$ is free from interference due to undesired symbols $\eta_{3,3}$ and $\eta_{4,1}$. Instead, it receives a noise-corrupted signal that depends on its desired symbol $\eta_{1,1}$. UE$_2$, on the other hand, observes a signal that depends solely on undesired symbols $\eta_{1,1},\eta_{3,3}$ and $\eta_{4,1}$ denoted by $I(\eta_{1,1},\eta_{3,3},\eta_{4,1})$ in Fig. \ref{fig:one_shot_M2_K2}. In the remaining $T_2$\footnote{In the schemes of corner points $\Big(\frac{1}{2},1\Big)$ and $\Big(\frac{1}{2},\frac{5}{4}\Big)$, $T_2$ corresponds to $1$ and $3$ channel uses, respectively.} channel uses, cooperative DeNB-RN zero-forcing is applied for the case when $M=K=2$ and simple RN unicasting when $M=2,K=1$.   

\subsubsection*{Decoding at the RNs and the UEs} As opposed to all prior schemes, RNs and UEs can decode each desired symbol on a single-channel use basis, i.e., symbol decoding over multiple channel uses is not required in attaining the optimal NDT. In consequence, channel diversity over multiple channel uses is not required.  

Specifically, in the proposed scheme for corner point $\Big(\frac{1}{2},1\Big)$, UE$_1$ decodes its $L_1=2$ desired symbols $\eta_{1,1}$ and $\eta_{1,2}$ in $T_1+T_2=2$ channel uses, namely, $1$ and $2$ (cf. Fig. \ref{fig:one_shot_M2_K1}), respectively. The RNs, on the contrary, only need the first channel use ($T_1=1$) to retrieve $L_1(1-\mu)=1$ desired symbols. In conclusion, this conforms to an NDT of $\frac{T_1+T_2}{L_1}=1$. 

In the other scheme, as shown in Fig. \ref{fig:one_shot_M2_K2}, UE$_1$ (UE$_2$) decodes its $L_2=4$ desired symbols $\eta_{1,1},\eta_{1,2},\eta_{1,3}$ and $\eta_{1,4}$ ($\eta_{2,1},\eta_{2,2},\eta_{2,3}$ and $\eta_{2,4}$) in 4 out of $T_1+T_2=5$ channel uses, namely, $1,2,3$ and $4$ ($4,5,2$ and $3$), respectively. Unlike the UEs, each RN only needs the first $T_1=2$ channel uses to retrieve its $L_2(1-\mu)=2$ desired symbols. Ultimately, the NDT becomes $\frac{T_1+T_2}{L_2}=\frac{5}{4}$. 

\subsection{Achievability for $M=13$}\label{subsec:ach_M3}

The optimal delivery-time cache-memory trade-off for $M=3$ and $K=1$ is presented. Hereby, the following proposition quantifies the achievable NDT.    

\begin{proposition}\label{prop_M3}
	The achievable NDT of the network under study for $M=3$ RNs, $K=1$ UEs and $\mu\in[0,1]$ is given by 
	\begin{equation}
	\label{eq:ach_NDT_M_3_K_1}
	\delta(\mu)=\max\Big\{1,4-9\mu\Big\}.
	\end{equation}
\end{proposition}

Similarly, to the achievability of corner points when $M=2$, it suffices to establish a scheme that attains an NDT of $1$ at $\mu=\frac{1}{3}$. The NDT-optimal scheme that establishes this result is the one-shot scheme of Section \ref{cha_one_shot}. Since the main idea of this scheme has already been illustrated through explicit examples for corner points $\Big(\frac{1}{2},1\Big)$ when $M=2,K=1$ and $\Big(\frac{1}{2},\frac{5}{4}\Big)$ when $M=2,K=2$, we omit further details for the sake of brevity. The interested reader can reconstruct the explicit scheme for $M=3$ and $K=1$ from the generalized scheme of Section \ref{cha_one_shot} for Region B.     
     

==> content/lw_bound__Anas_Chaaban_s_conflicted_copy_2017-12-28_.tex <==
\section{Lower Bound (Converse) of the Minimum NDT}
\label{sec:lw_bd}

In this section, we present the proof of the lower bound of the minimum NDT in Theorem \ref{theorem_lower_bound}. The method of the proof combines the approaches of \cite{avik} and \cite{conference214}.  

In the following, we expound the key idea of the proof. To this end, we introduce the following assumptions. First, we presume that all $K$ UEs and $M$ RNs request \emph{distinct} files $W_{d_j}$ ($d_j\neq d_\ell,j\neq \ell$). Second, without loss of generality, we assume that the requested files by the $K$ UEs are $W_{[1:K]}=(W_1,W_2,\ldots,W_K)$ and of the $M$ RNs $W_{[K+1:K+M]}=(W_{K+1},W_{K+2},\ldots,W_{K+M})$\footnote{Note that $K+M$ distinct files $W_{d_k}$ are available if there are at least as many files in the library, i.e., $N\geq K+M$.}. Under this demand pattern and given channel realizations $\mathbf{f},\mathbf{g}$ and $\mathbf{H}$, we obtain a lower bound on the delivery time $T=T(\mathbf{d},\mathbf{f},\mathbf{g},\mathbf{H})$, and therefore ultimately on the NDT, of any \emph{feasible} scheme.

The key idea in establishing the lower bound on the NDT is that $K+\ell$ requested files, comprising of all $K$ files $W_{[1:K]}$ requested by the UEs and $\ell$ files desired by a subset of $\ell$ RNs (out of $M$ RNs), e.g., $W_{[K+1:K+\ell]}$\footnote{For ease of notation, we assume that the $\ell$ files retrieved by the RNs are $W_{[K+1:K+\ell]}$. }, can be retrieved in the \emph{high SNR regime} from 

\begin{itemize}[leftmargin=*]
	\item $s$ output signals of the UEs, e.g., $\mathbf{y}^{T}_{u,[1:s]}$ for $1\leq s\leq \min\{M+1,K\}$, and
	\item $\ell$ cached contents of $\ell$ RNs, e.g., $S_{[1:\ell]}$, where $\bar{s}\leq\ell\leq M$ and $\bar{s}=M+1-s$. 
\end{itemize} We note that since $s+\ell\geq M+1$ holds, we are able to reconstruct all $M+1$ transmit signals ($x_s[t]$ and $x_{r,m}[t],m\in[M]$) at all $T$ time instants of the delivery phase within bounded noise. We start the converse as follows:
%\begin{eqnarray}\label{eq:conv_1}
%(K+\ell)L &= & H\big(W_{[1:K+\ell]}\big) \stackrel{(a)}= H\big(W_{[1:K+\ell]}|W_{[K+\ell+1:N]}\big) \nonumber \\
% &=&I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{[1:s]},S_{[1:\ell]}|W_{[K+\ell+1:N]}\big)+H\big(W_{[1:K+\ell]}|\mathbf{y}^{T}_{[1:s]},S_{[1:\ell]},W_{[K+\ell+1:N]}\big).
%\end{eqnarray} 
\begin{eqnarray}\label{eq:conv_1}
(K+\ell)L &= & H\big(W_{[1:K+\ell]}\big)= H\big(W_{[1:K+\ell]}|W_{[K+\ell+1:N]}\big) \nonumber \\
&=&I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]}|W_{[K+\ell+1:N]}\big)+H\big(W_{[1:K+\ell]}|\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]},W_{[K+\ell+1:N]}\big)
\end{eqnarray} In what follows, we upper bound each summand in Eq. \eqref{eq:conv_1} individually. The first summand is upper bounded according to:
%\begin{flalign}
%\label{eq:conv_term1}
%&I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]}|W_{[K+\ell+1:N]}\big)\nonumber\\&=I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)+I\big(W_{[1:K+\ell]};S_{[1:\ell]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\leq I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)+I\big(W_{[1:K+\ell]};S_{[1:\ell]},W_{[1:s]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&= I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)+I\big(W_{[1:K+\ell]};W_{[1:s]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\qquad+I\big(W_{[1:K+\ell]};S_{[1:\ell]}|W_{[1:s]\cup[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&= h\big(\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)-h\big(\mathbf{y}^{T}_{u,[1:s]}|W_{[1:N]}\big)+ H\big(W_{[1:s]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\qquad-H\big(W_{[1:s]}|W_{[1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)+ H\big(S_{[1:\ell]}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\qquad- H\big(S_{[1:\ell]}|W_{[1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\
%&\stackrel{(a)}\leq h\big(\mathbf{y}^{T}_{u,[1:s]}\big)-h\big(\mathbf{z}^{T}_{u,[1:s]}\big)+L\epsilon_L+ H\big(S_{[1:\ell]}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\stackrel{(b)}\leq sT\log(2\pi e(cP+1))-h\big(\mathbf{z}^{T}_{u,[1:s]}\big)+L\epsilon_L+\sum_{i=1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]},S_{[1:i-1]}\big)\nonumber\\&\stackrel{(c)}= sT\log(cP+1)+L\epsilon_L+\sum_{i=1}^{\bar{s}}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\leq sT\log(cP+1)+L\epsilon_L+\sum_{i=1}^{\bar{s}}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]}\big)+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\leq sT\log(cP+1)+L\epsilon_L+\sum_{i=1}^{\bar{s}}\sum_{j=s+1}^{K+\ell}H\big(S_{i,j}\big)+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\stackrel{(d)}\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\stackrel{(e)}= sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]},\mathbf{x}_{r,[1:i-1]}[1]\big)\nonumber\\&\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L\nonumber\\&+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i},W_{[s+1:K+i-1]},\mathbf{z}^{T}_{u,[1:K]},\mathbf{z}^{T}_{r,[1:i-1]}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]},\mathbf{x}_{r,[1:i]}[1]\big)\nonumber\\&\stackrel{(f)}\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+\sum_{i=\bar{s}+1}^{\ell}T(K+i-1)\log(2\pi e)\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}H\big(W_{[s+1:K+i-1]}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]},\mathbf{x}_{r,[1:i]}[1],,\mathbf{z}^{T}_{u,[1:K]},\mathbf{z}^{T}_{r,[1:i-1]}\big)\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}H\big(S_i|W_{[1:K+i-1]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]},\mathbf{x}_{r,[1:i]}[1],,\mathbf{z}^{T}_{u,[1:K]},\mathbf{z}^{T}_{r,[1:i-1]}\big)\nonumber\\&\stackrel{(g)}\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+\Bigg[T\bigg((K-1)(\ell-\bar{s})+\frac{\ell(\ell+1)}{2}-\frac{\bar{s}(\bar{s}+1)}{2}\bigg)\Bigg]\log(2\pi e)\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}\sum_{j=K+i}^{K+\ell}H\big(S_{i,j}\big)\nonumber\\&\stackrel{(d)}\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+\Bigg[T\bigg((K-1)(\ell-\bar{s})+\frac{\ell(\ell+1)}{2}-\frac{\bar{s}(\bar{s}+1)}{2}\bigg)\Bigg]\log(2\pi e)\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}(\ell-i+1)\mu L\nonumber\\&= sT\log(cP+1)+L\epsilon_L+\Bigg[T\bigg((K-1)(\ell-\bar{s})+\frac{\ell(\ell+1)}{2}-\frac{\bar{s}(\bar{s}+1)}{2}\bigg)\Bigg]\log(2\pi e)\nonumber\\&\quad+\Bigg[\bar{s}\bigg(K-s+\frac{\bar{s}-1}{2}\bigg)+\frac{\ell(\ell+1)}{2}\Bigg]\mu L,\end{flalign} 
\begin{flalign}
\label{eq:conv_term1}
&I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]}|W_{[K+\ell+1:N]}\big)\nonumber\\&=I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)+I\big(W_{[1:K+\ell]};S_{[1:\ell]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\leq I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)+I\big(W_{[1:K+\ell]};S_{[1:\ell]},W_{[1:s]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&= I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)+I\big(W_{[1:K+\ell]};W_{[1:s]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\qquad+I\big(W_{[1:K+\ell]};S_{[1:\ell]}|W_{[1:s]\cup[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&= h\big(\mathbf{y}^{T}_{u,[1:s]}|W_{[K+\ell+1:N]}\big)-h\big(\mathbf{y}^{T}_{u,[1:s]}|W_{[1:N]}\big)+ H\big(W_{[1:s]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\qquad-H\big(W_{[1:s]}|W_{[1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)+ H\big(S_{[1:\ell]}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\qquad- H\big(S_{[1:\ell]}|W_{[1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\
&\stackrel{(a)}\leq h\big(\mathbf{y}^{T}_{u,[1:s]}\big)-h\big(\mathbf{z}^{T}_{u,[1:s]}\big)+L\epsilon_L+ H\big(S_{[1:\ell]}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}\big)\nonumber\\&\stackrel{(b)}\leq sT\log(2\pi e(cP+1))-h\big(\mathbf{z}^{T}_{u,[1:s]}\big)+L\epsilon_L+\sum_{i=1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]},S_{[1:i-1]}\big)\nonumber\\&\stackrel{(c)}= sT\log(cP+1)+L\epsilon_L+\sum_{i=1}^{\bar{s}}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\leq sT\log(cP+1)+L\epsilon_L+\sum_{i=1}^{\bar{s}}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]}\big)+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\leq sT\log(cP+1)+L\epsilon_L+\sum_{i=1}^{\bar{s}}\sum_{j=s+1}^{K+\ell}H\big(S_{i,j}\big)+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\stackrel{(d)}\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]}\big)\nonumber\\&\stackrel{(e)}= sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]},\mathbf{x}_{r,[1:i-1]}[1],\mathbf{z}^{T}_{u,[s+1:K]},\mathbf{z}^{T}_{r,[1:i-1]}\big)\nonumber\\&\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L\nonumber\\&+\sum_{i=\bar{s}+1}^{\ell}H\big(S_{i},W_{[s+1:K+i-1]}|W_{[1:s]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]},\mathbf{x}_{r,[1:i]}[1],\mathbf{z}^{T}_{u,[s+1:K]},\mathbf{z}^{T}_{r,[1:i-1]}\big)\nonumber\\&\stackrel{(f)}\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+To(\log(P))\nonumber\\&\quad+\sum_{i=\bar{s}+1}^{\ell}H\big(S_i|W_{[1:K+i-1]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{u,[1:s]}, S_{[1:i-1]},\mathbf{x}_{r,[1:i]}[1],\mathbf{z}^{T}_{u,[s+1:K]},\mathbf{z}^{T}_{r,[1:i-1]}\big)\nonumber\\&\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+To(\log(P))+\sum_{i=\bar{s}+1}^{\ell}\sum_{j=K+i}^{K+\ell}H\big(S_{i,j}\big)\nonumber\\&\stackrel{(d)}\leq sT\log(cP+1)+L\epsilon_L+\bar{s}(K+\ell-s)\mu L+To(\log(P))+\sum_{i=\bar{s}+1}^{\ell}(\ell-i+1)\mu L\nonumber\\&= sT\log(cP+1)+L\epsilon_L+To(\log(P))+\Bigg[\bar{s}\bigg(K-s+\frac{\bar{s}-1}{2}\bigg)+\frac{\ell(\ell+1)}{2}\Bigg]\mu L,\end{flalign} 
where the steps in \eqref{eq:conv_term1} are explained as follows:
\begin{itemize}
	\item Step (a) follows from the fact that dropping the conditioning on the first term does not increase entropy. Further, we apply Fano's inequality to the third term. Hereby, $\epsilon_L$ is a function, independent of $P$ which vanishes in the limit as $L\rightarrow\infty$. 
	\item Step (b) follows by applying \cite[Lemma 1]{avik} on the first differential entropy term. Additionally, we use the chain rule to rewrite the fourth term. 
	\item Step (c) is due to the fact that the channel noise $\mathbf{z}^{T}_{u,[1:s]}$ is i.i.d. across time and has a Gaussian distribution with zero mean and unit variance. 
	\item Step (d) is since the entropy of each local file cache content is upper bounded according to $H(S_{ij})\leq\mu L$.   
	\item In step (e), we use the fact that in the first channel use ($t=1$), the transmit signal $x_{r,m}[1]$ at RN$_m$ depends (apart from CSI) solely on the cached content $S_m$. Further, we note that the noise terms $\mathbf{z}^{T}_{u,[s+1:K]}$ and $\mathbf{z}^{T}_{r,[1:i-1]}$ are independent of all the remaining random variables in the conditional entropy term.  
	\item Step (f) follows from \cite[Lemma 2]{avik}. In the nutshell, this lemma states that the files $W_{[s+1:K+i-1]}$ can be resolved from $S_{[1:i-1]}$ and $\mathbf{y}^{T}_{u,[1:s]}$ (if $i-1+s\geq M+1$) within bounded noise distortion $To(\log(P))$, where $o(\log(P))\rightarrow 0$ as $P\rightarrow\infty$. This works since the following Markov chains are applicable to the network:
	\newline
	\vspace{-2em}
	\begin{enumerate}[leftmargin=3\parindent] 
		\item[1a)] $S_{[1:i-1]}\rightarrow\mathbf{x}_{r,[1:i-1]}[1]$  
		\item[1b)] $\big(S_{[1:i-1]},\mathbf{y}_{r,[1:i-1]}[t]\big)\rightarrow\mathbf{x}_{r,[1:i-1]}[t],\forall t\in[2:T]$ 
		\item[2)] $\big(\mathbf{x}_{r,[1:i-1]}[t],\mathbf{y}_{u,[1:s]}[t],\mathbf{z}_{u,[1:K]}[t],\mathbf{z}_{r,[1:i-1]}[t]\big)\rightarrow\big(\mathbf{y}_{u,[s+1:K]}[t],\mathbf{y}_{r,[1:i-1]}[t]\big)$ if $i-1\geq\bar{s}\triangleq M+1-s,\forall t\in[T]$
		\item[3a)]
		$\mathbf{y}^{T}_{u,[s+1:K]}\rightarrow W_{[s+1:K]}$
		\item[3b)]
		$\Big(\mathbf{y}^{T}_{r,[1:i-1]},S_{[1:i-1]}\Big)\rightarrow W_{[K+1:K+i-1]}$   	
	\end{enumerate}	  
\end{itemize}

Next, we use the aforementioned steps $(a),(e)$ and $(f)$, respectively, to upper bound the second summand of Eq. \eqref{eq:conv_1}.
\begin{flalign}
\label{eq:conv_term2}
&H\big(W_{[1:K+\ell]}|\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]},W_{[K+\ell+1:N]}\big)\nonumber\\&=H\big(W_{[1:s]}|\mathbf{y}^{T}_{u,[1:s]}\big)+H\big(W_{[s+1:K]}|\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]},W_{[1:s]\cup[K+\ell+1:N]}\big)\nonumber\\&\quad+H\big(W_{[K+1:K+\ell]}|\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]},W_{[1:K]\cup[K+\ell+1:N]}\big)\nonumber\\&\stackrel{(a)}\leq L\epsilon_L+H\big(W_{[s+1:K]}|\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]},W_{[1:s]\cup[K+\ell+1:N]}\big)+H\big(W_{[K+1:K+\ell]}|\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]},W_{[1:K]\cup[K+\ell+1:N]}\big)\nonumber\\&\stackrel{(e)}= L\epsilon_L+H\big(W_{[s+1:K]}|\mathbf{y}^{T}_{u,[1:s]},\mathbf{z}^{T}_{u,[s+1:K]},\mathbf{z}^{T}_{r,[1:i-1]},S_{[1:\ell]},\mathbf{x}_{r,[1:\ell]}[1],W_{[1:s]\cup[K+\ell+1:N]}\big)\nonumber\\&\quad+H\big(W_{[K+1:K+\ell]}|\mathbf{y}^{T}_{u,[1:s]},\mathbf{z}^{T}_{u,[s+1:K]},\mathbf{z}^{T}_{r,[1:i-1]},S_{[1:\ell]},\mathbf{x}_{r,[1:\ell]}[1],W_{[1:K]\cup[K+\ell+1:N]}\big)\nonumber\\&\stackrel{(f)}\leq L\epsilon_L+T o(\log(P)) 
\end{flalign} 

Combining \eqref{eq:conv_term1} and \eqref{eq:conv_term2} in \eqref{eq:conv_1}, we get the following inequality
\begin{align}
\label{eq:ineq_bound}
(K+\ell)L\leq sT\log(cP+1)+\Bigg[\bar{s}\bigg(K-s+\frac{\bar{s}-1}{2}\bigg)+\frac{\ell(\ell+1)}{2}\Bigg]\mu L+L\epsilon L+To(\log(P))
\end{align}
Dividing both sides of \eqref{eq:ineq_bound} by $L$, letting $L\rightarrow\infty$ and $P\rightarrow\infty$, we obtain the following class of lower bounds on the minimum NDT
\begin{align}\label{eq:delta_lb_bound}
\delta^{\star}(\mu)\geq\delta_{\text{LB}}(\mu,\ell,s)\triangleq\frac{K+\ell-\mu(\bar{s}\big(K-s+\frac{(\bar{s}-1)}{2}\big)+\frac{\ell}{2}(\ell+1))}{s}.
\end{align} By optimizing the bound $\delta_{\text{LB}}(\mu,\ell,s)$ in \eqref{eq:delta_lb_bound} with respect to $\ell\in[\bar{s}:M]$ and $s\in[\min\{M+1,K\}]$, we determine one term of the NDT lower bound in \eqref{eq:NDT_lw_bound}. Additionally, we recall that the NDT is also bounded from below by the performance of the reference interference-free system which has an NDT of $1$. The maximum over these two lower bounds concludes the proof of Theorem \ref{theorem_lower_bound}.     

%=H\big(W_{[1:K+\ell]}|\mathbf{y}^{T}_{u,[1:s]},S_{[1:\ell]},\mathbf{x}_{r,[1:\ell]}[1],W_{[K+\ell+1:N]}\big)\nonumber
  
%\vspace{3em}
%
%An other way of bounding $T$ applicable for $0\leq\ell\leq M$ and $p_\ell=\min\{M-\ell,K\}$ can be conducted as follows:
%
%\begin{eqnarray}\label{eq:conv_2}
%(K+\ell)L &= & H\big(W_{[1:K+\ell]}\big) \stackrel{(a)}= H\big(W_{[1:K+\ell]}|W_{[K+\ell+1:N]}\big) \nonumber \\
% &=&I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}, \nonumber\\&&\qquad\quad S_{[1:\ell]}|W_{[K+\ell+1:N]}\big)\nonumber \\&+&H\big(W_{[1:K+\ell]}|\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}, \nonumber\\&&\qquad\quad S_{[1:\ell]},W_{[K+\ell+1:N]}\big).\nonumber
%\end{eqnarray}
%
%We bound the mutual information term according to:
%
%\begin{flalign}
%\label{eq:conv_term_bound_2}
%&I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1},S_{[1:\ell]}|W_{[K+\ell+1:N]}\big)\nonumber\\&=I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}|W_{[K+\ell+1:N]}\big)\nonumber\\&\qquad+I\big(W_{[1:K+\ell]};S_{[1:\ell]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&\stackrel{(a)}\leq I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}|W_{[K+\ell+1:N]}\big)\nonumber\\&\qquad+I\big(W_{[1:K+\ell]};S_{[1:\ell]},W_{[1:p_\ell]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&= I\big(W_{[1:K+\ell]};\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}|W_{[K+\ell+1:N]}\big)\nonumber\\&\qquad+I\big(W_{[1:K+\ell]};W_{[1:p_\ell]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&\qquad+I\big(W_{[1:K+\ell]};S_{[1:\ell]}|W_{[1:p_\ell]\cup[K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&= h\big(\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}|W_{[K+\ell+1:N]}\big)\nonumber\\&\qquad-h\big(\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}|W_{[1:N]}\big)\nonumber\\&\qquad+ H\big(W_{[1:p_\ell]}|W_{[K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&\qquad- H\big(W_{[1:p_\ell]}|W_{[1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&\qquad+ H\big(S_{[1:\ell]}|W_{[1:p_\ell]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&\qquad- H\big(S_{[1:\ell]}|W_{[1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\
%&\stackrel{(b)}\leq h\big(\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)-h\big(\mathbf{z}^{T}_{[1:K]}\big)+L\epsilon_L\nonumber\\&\qquad+ H\big(S_{[1:\ell]}|W_{[1:p_\ell]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1}\big)\nonumber\\&\stackrel{(c)}\leq (p_\ell+1) T\log(2\pi eP)+L\epsilon_L\nonumber\\&\qquad+\sum_{i=1}^{\ell}H\big(S_{i}|W_{[1:p_\ell]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1},S_{[1:i-1]}\big)\nonumber\\&\stackrel{(d)}= (p_\ell+1) T\log(2\pi eP)+L\epsilon_L\nonumber\\&\quad+\sum_{i=1}^{\ell}H\big(S_{i}|W_{[1:p_\ell]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{z}^{T}_{r,[1:i-1]},\nonumber\\&\qquad\qquad\mathbf{x}^{T}_{M+1},\mathbf{x}^{T}_{[1:i-1]} S_{[1:i-1]}\big)\nonumber\\&\stackrel{(e)}\leq (p_\ell+1)T\log(2\pi eP)+L\epsilon_L\nonumber\\&\quad+\sum_{i=1}^{\ell}H\big(S_{i}|W_{[1:p_\ell]\cup [K+1:K+i-1]\cup [K+\ell+1:N]}\big)\nonumber\\&\stackrel{(f)}\leq (p_\ell+1)T\log(2\pi eP)+L\epsilon_L\nonumber\\&\quad+\sum_{i=1}^{\ell}(K-p_\ell+\ell-i+1)\mu L\nonumber\\&\stackrel{(g)}= (p_\ell+1)T\log(2\pi eP)+L\epsilon_L\nonumber\\&\quad+\ell (K-p_\ell+\nicefrac{(\ell+1)}{2})\mu L\nonumber
%\\&\stackrel{(f)}\leq qT\log(2\pi e\Lambda P)+L\epsilon_L+\min\{(K-q+\ell)(\bar{q}+1)\mu,K-q+\ell\}L\nonumber\\&\quad+\sum_{i=\bar{q}+2}^{\ell}H\big(S_{i}|W_{[1:q]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{[1:q]},\mathbf{z}^{T}_{[1:K]}, S_{[1:i-1]},\nonumber\\&\qquad\qquad\quad\mathbf{z}^{T}_{r,[1:i-1]},\mathbf{x}_{[1:\bar{q}+1}[1]\big)\nonumber\\&\stackrel{(g)}\leq qT\log(2\pi e\Lambda P)+L\epsilon_L+\min\{(K-q+\ell)(\bar{q}+1)\mu,K-q+\ell\}L\nonumber\\&\quad+\sum_{i=\bar{q}+2}^{\ell}H\big(S_{i}|W_{[1:q]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{[q+1:K]}, \mathbf{y}^{T}_{r,[1:i-1]}, S_{[1:i-1]}\big)\nonumber\\&\stackrel{(h)}\leq qT\log(2\pi e\Lambda P)+L\epsilon_L+\min\{(K-q+\ell)(\bar{q}+1)\mu,K-q+\ell\}L\nonumber\\&\quad+\sum_{i=\bar{q}+2}^{\ell}H\big(S_{i},W_{[q+1:K+i-1]}|W_{[1:q]\cup [K+\ell+1:N]},\mathbf{y}^{T}_{[q+1:K]},\mathbf{y}^{T}_{r,[1:i-1]},\nonumber\\&\qquad\qquad\quad S_{[1:i-1]}\big)\nonumber\\&\stackrel{(i)}\leq qT\log(2\pi e\Lambda P)+L\epsilon_L+\min\{(K-q+\ell)(\bar{q}+1)\mu,K-q+\ell\}L\nonumber\\&\quad+\sum_{i=\bar{q}+2}^{\ell}(\ell-i+1)\mu L\nonumber\\&\stackrel{(j)}\leq qT\log(2\pi e\Lambda P)+L\epsilon_L+\min\{(K-q+\ell)(\bar{q}+1)\mu,K-q+\ell\}L\nonumber\\&\quad+(\ell+1)(\nicefrac{\ell}{2}-\bar{q}-1)\mu L+\nicefrac{1}{2}(\bar{q}+1)(\bar{q}+2)\mu L
%\end{flalign}
%
%It can be readily seen that:
%\begin{flalign}
%% \label{eq:conv_term2_bound2}
%&H\big(W_{[1:K+\ell]}|\mathbf{y}^{T}_{[1:p_\ell]},\mathbf{z}^{T}_{[1:K]},\mathbf{x}^{T}_{M+1},S_{[1:\ell]},W_{[K+\ell+1:N]}\big)\nonumber\\&\leq L\epsilon_L
%\end{flalign}   
%\vspace{3em}
 
%\vspace{.5em}
%\begin{lemma}\label{lemma_lower_bound}
%For the transceiver cache-aided network with one DeNB, $M$ RNs each endowed with a cache of fractional cache size $\mu\in[0,1]$, $K$ UEs and a file library of $N\geq M+K$ files, the NDT is lower bounded under perfect CSI at all nodes by
%%\begin{align}\label{eq:NDT_lw_bound}
%%\delta^{\star}&(\mu)\geq\max\Bigg\{1,\nonumber\\&\max_{\substack{\ell\in[\bar{s}:M],\\s\in[\min\{M+1,K\}]\\\bar{s}=M+1-s}}\frac{K+\ell-\mu\Big(\bar{s}\big(K-s+\nicefrac{(\bar{s}-1)}{2}\big)+\nicefrac{\ell}{2}(\ell+1)\Big)}{s}\Bigg\}.
%%\end{align}  
%\begin{align}\label{eq:NDT_lw_bound}
%\delta^{\star}&(\mu)\geq\max\Big\{1,\max_{\substack{\ell\in[\bar{s}:M],\\s\in[\min\{M+1,K\}]}}\delta_{\text{LB}}(\mu,\ell,s)\Big\},
%\end{align} where $\bar{s}=M+1-s$ and 
%\begin{align}\label{eq:NDT_lw_bound_inner_comp}
%&\hspace{-.25cm}\delta_{\text{LB}}(\mu,\ell,s)=\frac{K+\ell-\mu(\bar{s}\big(K-s+\frac{(\bar{s}-1)}{2}\big)+\frac{\ell}{2}(\ell+1))}{s}.
%\end{align}
%\end{lemma}
%\begin{proof}
%The key idea behind the proof is provided in the previous paragraph. Details are omitted for the sake of brevity.
%\end{proof}

==> content/main_res__Jaber_Kakar_s_conflicted_copy_2018-01-15_.tex <==
\section{Main Results}
\label{sec:main_res}

In this section, we state our main results on the minimum NDT for the cache-enabled \alert{broadcast-relay} wireless network of Fig. \ref{fig:HetNet} for $M$ RNs and $K$ UEs. Hereby, our main results are presented in Theorems \ref{theorem_lower_bound}--\ref{th:one_shot_ach_NDT}. \alert{They include, respectively, a novel lower bound, an upper bound (achievability) on the NDT and a complete NDT-tradeoff characterization for $K+M\leq 4$.} Further, we formulate multiple corollaries that evaluate the performance of the scheme presented in Theorem \ref{th:one_shot_ach_NDT} with respect to the lower bound of Theorem \ref{theorem_lower_bound}.   

\begin{theorem}[Lower bound on NDT]\label{theorem_lower_bound}
	For the transceiver cache-aided network with one DeNB, $M$ RNs each endowed with a cache of fractional cache size $\mu\in[0,1]$, $K$ UEs and a file library of $N\geq K+M$ files, the optimal NDT is lower bounded under perfect CSI at all nodes by
	\begin{align}\label{eq:NDT_lw_bound}
	\delta^{\star}&(\mu)\geq\max\Big\{1,\max_{\substack{\ell\in[\bar{s}:M],\\s\in[\min\{M+1,K\}]}}\delta_{\text{LB}}(\mu,\ell,s)\Big\},
	\end{align} where $\bar{s}=M+1-s$ and 
	\begin{align}\label{eq:NDT_lw_bound_inner_comp}
	&\hspace{-.25cm}\delta_{\text{LB}}(\mu,\ell,s)=\frac{K+\ell-\mu(\bar{s}\big(K-s+\frac{(\bar{s}-1)}{2}\big)+\frac{\ell}{2}(\ell+1))}{s}.
	\end{align}
\end{theorem}
\begin{proof}
	The proof of Theorem \ref{theorem_lower_bound} will be given in Section \ref{sec:lw_bd}. \alert{To provide some insight into the lower bound presented in Theorem \ref{theorem_lower_bound}, however, we outline a short sketch of the proof. Particularly, we summarize the ideas when deriving the two terms in Eq. \eqref{eq:NDT_lw_bound}.} 
		
	\alert{First, we find the bound $\delta_{\text{LB}}(\mu,\ell,s)$ by exploiting the following main observation in the high SNR regime (where noise becomes negligible). That is, given the channel outputs of any $s$ UEs (e.g., of UE$_1$, UE$_2$, $\ldots$, UE$_s$ denoted by $\mathbf{y}_{u,[1:s]}^{T}$),} in addition to the cached content of $\ell$ RNs \alert{(e.g, cached contents of RN$_1$, RN$_2$, $\ldots$, RN$_\ell$ represented by $S_{[1:\ell]}$)} such that $s+\ell\geq M+1$ enables the decoding of all $K$ files requested by the UEs as well as $\ell$ files desired by the RNs. This is due to the fact that with this information set, all $M+1$ transmit signals \alert{consisting of} the DeNB signal $x_s$ and the RNs transmit signals $x_{r,m},\forall m\in[M]$, can be reproduced. This in turn, allows the reconstruction of the following channel outputs: On the one hand, the remaining $K-s$ channel outputs of the UEs and on the other hand $\ell$ outputs of the RNs. With the availability of $K$ UE channel ouputs as well $\ell$ RN channel outputs and cached contents, $K+\ell$ files in total become decodable. 
	
	\alert{Second, the unity lower bound follows from the fact that the NDT is bounded from below by the performance of the reference interference-free system with an NDT of $1$}. The maximum over these two lower bounds concludes the proof of Theorem \ref{theorem_lower_bound}.                 
\end{proof}

Before establishing the achievability at fractional cache sizes in the range $\mu\in(0,1)$, we consider two special corner points at fractional cache sizes $\mu=0$ and $\mu=1$ for \emph{arbitrary} $M$ and $K$. These are the cases where the RN has either \emph{zero-cache} ($\mu=0$) or \emph{full-cache} ($\mu=1$) capabilities. In the following lemma, we expound the \emph{optimal NDT} for these two points.  
\vspace{.5em}
\begin{lemma}\label{corr_mu_0_and_1}
	For the transceiver cache-aided network with one DeNB, $M$ RNs each endowed with a cache of fractional cache size $\mu$, $K$ UEs and a file library of $N\geq M+K$ files, the optimal NDT is
	\begin{equation}\label{eq:opt_NDT_mu_0}
	\delta^{\star}(\mu)=K+M\:\:\text{ for }\mu=0,
	\end{equation} 
	achievable via DeNB broadcasting to $M$ RNs and $K$ UEs, and 
	\begin{equation}
	\label{eq:opt_NDT_mu_1}
	\delta^{\star}(\mu)=\max\Bigg\{1,\frac{K}{M+1}\Bigg\}\:\:\text{ for }\mu=1,
	\end{equation} 
	achievable via zero-forcing beamforming for an $(M+1,K)$ MISO\footnote{In MISO broadcast channels, we use the notation, $(a,b)$ for integers $a$ and $b$ to denote a broadcast channel with $a$ transmit antennas and $b$ single antenna receivers.} broadcast channel. 
\end{lemma}
\begin{proof}
	For the proof, it suffices to find a cache transmission policy that matches the lower bound in Thoerem \ref{theorem_lower_bound} for $\mu=0$ and $\mu=1$, respectively. On the one hand, if $\mu=0$, we note that $\delta_{\text{LB}}(0,M,1)=K+M$. On the other hand, if $\mu=1$, we observe that $\delta_{\text{LB}}(1,0,M+1)=\nicefrac{K}{(M+1)}$ if $M+1\leq K$ and $\delta_{\text{LB}}(1,\ell,s)<1$ if $M+1>K$. Next, we consider the achievability at $\mu=0$ and $\mu=1$. For these two fractional cache sizes, the network in Fig. \ref{fig:HetNet} reduces to a SISO broadcast channel (BC) with $K+M$ users for $\mu=0$ and an $(M+1,K)$ MISO broadcast channel for $\mu=1$. The approximate \emph{per-user} rate (neglecting $o(\log(P))$ bits) for these two channels are known to be $\frac{1}{(K+M)}\log(P)$ \cite{Jafar07} (achievable through unicasting each user's message) \alert{for $\mu=0$} and $\frac{1}{K}\min\{M+1,K\}\log(P)$ (achievable through zero-forcing beamfoming) \cite{Weingarten06} \alert{for $\mu=1$}, respectively. Equivalently, each user needs the reciprocal per-user rate of signaling dimensions (e.g., channel uses in time) %or frequency) 
	to retrieve one desired bit \alert{reliably}. Thus, the approximate DTB becomes, respectively, $\frac{(K+M)}{\log(P)}$ and $\frac{K}{\min\{M+1,K\}\log(P)}$. Normalizing the delivery time per bit by the point-to-point reference DTB $\frac{1}{\log(P)}$ generates the NDTs $K+M$ and $\max\{1,\nicefrac{K}{(M+1)}\}$. This establishes the NDT-optimality at these fractional cache sizes.
\end{proof}
%\vspace{.5em}
\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.475\textwidth}
		\centering
		\begin{tikzpicture}[scale=0.8]
		\PlotNDTMOneKOne
		\end{tikzpicture}
		\caption[NDT for $M=K=1$]{\small NDT for $M=K=1$}
		\label{fig:NDT_M_K_1_1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.475\textwidth}  
		\centering 
		\begin{tikzpicture}[scale=0.8]
		\PlotNDTMOneKTwo
		\end{tikzpicture}
		\caption[NDT for $M=1,K=2$]{\small NDT for $M=1, K=2$} 
		\label{fig:NDT_M_K_1_2}       
	\end{subfigure}
	\caption[NDT as a function of $\mu$ for $M=1$ and $K\leq 2$]
	{\small Optimal NDT as a function of $\mu$ for $M=1$ and $K\leq 2$} 
	\label{fig:NDT_M_K_1_LEQ_2}
\end{figure*} 
\begin{remark}
	From Lemma \ref{corr_mu_0_and_1}, we infer that the caching problem for the system illustrated in Fig. \ref{fig:HetNet} establishes the behavior of the network in terms of delivery time between the two extremes -- SISO BC with $K+M$ users and an $(M+1,K)$ MISO BC. This analysis will reveal what kind of schemes other than simple unicasting and zero-forcing will be optimal for $0<\mu<1$.
\end{remark}
\begin{remark}[\alert{Optimality of Memory Sharing of Zero-cache and Full-cache Schemes}]\label{remark:memory_sharing_opt}\alert{Memory sharing of optimal schemes at extreme points of zero-cache ($\mu=0$) and full-cache ($\mu=1$) may be optimal. Or in other words, the optimal NDT of intermediate points at fractional cache sizes $0<\mu<1$ may be achievable through successively time-sharing between unicasting and zero-forcing on $(1-\mu)$ and $\mu$ fractions of the files, respectively. This scheme suggests treating uncached and cached file fractions \emph{independently} by applying two \emph{separate} delivery schemes -- unicasting and zero-forcing. However, as shown in Fig. \ref{fig:NDT_M_K_1_LEQ_2}, this only happens for cases where $M=1$ and $K\leq 2$. In these cases, the lower bound $\delta_{\text{LB}}(\mu,1,1)$ coincides with the achievable NDT. Intuitively, this result makes sense because of the following two reasons. On the one hand, when $M=1$, there are (with respect to $(1-\mu)$ fractions of uncached information on each file) (i) no multicasting opportunities on the DeNB-RN broadcast channel and (ii) no zero-forcing opportunities on the RN-UE channel. On the other hand, when $K\leq 2$ joint DeNB-RN zero-forcing beamforming guarantees (with respect to the cached fractions of the files all $K$ UEs desire) that every UE receives in \emph{each} channel use desired information on its requested file since $K\leq M+1=2$. Thus, in conclusion, for these cases applying unicasting and joint DeNB-RN beamforming successively on $(1-\mu)$ and $\mu$ file fractions is NDT-optimal. However, this is in general not true for arbitrary instances of $K$ and $M$ as we shall see next.}            
\end{remark}
\alert{In Remark \ref{remark:memory_sharing_opt}, we have discussed cases where successively applying unicasting and joint DeNB-RN beamforming on uncached and cached file fractions is NDT-optimal at fractional cache sizes $0<\mu<1$. However, in general, (with the exception of $M=1, K\leq 2$) delivery schemes that treat uncached and cached file fractions independently are \emph{sub-optimal} for arbitrary $K$ and $M$. To this end, we propose a general \emph{one-shot} (OS) scheme that treats uncached and cached file fractions \emph{jointly} by exploiting multicasting and zero-forcing opportunities. Our proposed one-shot scheme is with the exception of the full-duplex requirement at the RNs simple in implementation because all receiving nodes are able to decode their \emph{desired} symbols on a \emph{single} channel use basis. In other words, these schemes explicitly preclude symbol decoding over multiple channel uses. The next theorem specifies the achievable NDT for these one-shot schemes.}       
\vspace{.5em}
\begin{theorem}[Achievable One-Shot NDT]\label{th:one_shot_ach_NDT}
	For $N\geq K+M$ files, $K$ UEs and $M$ RNs each with a cache of (fractional) size $\mu\in\{0,\nicefrac{1}{M},\nicefrac{2}{M},\nicefrac{3}{M},\ldots,\nicefrac{(M-1)}{M},1\}$,
	%\begin{align}\label{eq:NDT_OS_ach}
	%\delta^{\star}(\mu)\leq\delta_{\text{OS}}(\mu)\triangleq\max\Bigg\{\delta_{\text{MAN}}(\mu),\frac{K+\delta_{\text{MAN}}(\mu)\boldsymbol{1}_{K>\mu M}}{\min\{K,1+\mu M\}}\Bigg\}
	%\end{align} 
	\begin{align}\label{eq:NDT_OS_ach}
	\delta_{\text{OS}}(\mu)\triangleq\max\Bigg\{\delta_{\text{MAN}}(\mu),\frac{K+\delta_{\text{MAN}}(\mu)\boldsymbol{1}_{K>\mu M}}{\min\{K,1+\mu M\}}\Bigg\}
	\end{align} is achievable, where $\boldsymbol{1}_{K>\mu M}$ is the indicator function and $\delta_{\text{MAN}}(\mu)$ is the achievable Maddah-Ali Niesen (MAN) NDT given by
	\begin{equation*}
	\delta_{\text{MAN}}(\mu)=M\cdot(1-\mu)\cdot\frac{1}{1+\mu M} 
	\end{equation*} such that $\delta^{\star}(\mu)\leq\delta_{\text{OS}}(\mu)$. For arbitrary $\mu\in[0,1]$, the lower convex envelope of these points is achievable.  
\end{theorem}
\begin{proof}
	Details on the scheme are presented in Section \ref{cha_one_shot}. Nevertheless, we use this paragraph to highlight the main idea of the scheme. \alert{Recall that the file length is denoted by $L$.} \alert{The scheme we develop (potentially) consists of two phases requiring $T_1$ and $T_2$ channel uses, respectively, to send uncached $(1-\mu)L$ Gaussian symbols (each symbol carrying approximately $\log(P)$ bits) to each RN and also $L$ symbols to each UE}. 
	
	In every channel use of the \emph{first phase} \alert{depicted in Fig. \ref{fig:OS_Phase1}, beamforming facilitates combining the MAN scheme \cite{Maddah-Ali2} with zero-forcing beamforming to (i) pre-cancel interference caused by applying on the DeNB-RN broadcast channel and (ii) convey desired symbols to UEs. Precisely, the MAN scheme is applied on the DeNB-RN broadcast channel} to provide each RN in a subset $\mathcal{S}_R\subset[M]$ \alert{with} $|\mathcal{S}_R|=1+\mu M$ RNs with a desired symbol. \emph{Simultaneously}, the full-duplex capabilities at the RN is exploited by conveying \alert{to} each UE in the subset $\mathcal{S}_U\subset[K]$ \alert{with} $|\mathcal{S}_U|=\min\{K,\mu M\}$ UEs in total with a desired symbol by zero-forcing the contribution of all interfering symbols that $|\mathcal{S}_R|=1+\mu M$ RNs in $\mathcal{S}_R$ desire. \alert{Recall that the first phase consumes $T_1$ channel uses. We show that $T_1$ channel uses suffice in sending each RN$_m$, $\forall m\in[M]$, the remaining $(1-\mu)L$ bits of its requested file. Simultaneously, in $T_1$ channel uses each UE$_k$, $\forall k\in[K]$, receives $\tilde{L}$ symbols of its desired symbol, with $\tilde{L}$ being proportional to $|\mathcal{S}_U|=\min\{K,\mu M\}$. Thus, we may encounter cases where it is either feasible or infeasible to communicate all $L$ symbols of each requested file to the respective UEs in $T_1$ channel uses ($\tilde{L}\geq L$ or $\tilde{L}<L$).}    
	
	\alert{Only in the case of missing symbols ($\tilde{L}<L$) that all $K$ UEs still require after $T_1$ channel uses, additional $T_2>0$ channel uses are required in phase two to deliver the remaining desired symbols as shown in Fig. \ref{fig:OS_Phase2}.} To this end, in every channel use \emph{cooperative DeNB-RN zero-forcing beamforming} is deployed to send one symbol in total to $\psi'=\min\{K,1+\mu M\}$ UEs. The decoding at the RNs and UEs does not involve symbol decoding over multiple channel uses. Instead, decoding occurs on a one-shot, or single channel use, basis. In conclusion, the achievable NDT becomes either $\frac{T_1}{L}$ if \alert{$T_2=0$} or $\frac{T_1+T_2}{L}$ if \alert{$T_2>0$} with $L$ being the file size.     
\end{proof}

\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.475\textwidth}
		\centering
		\vspace{10.5em}
		\begin{tikzpicture}[scale=1]
		\SymModSchemePhaseOne
		\end{tikzpicture}
		\vspace{-14em}
		\caption{\small Scheme for the first phase ($t\in[T_1]$) with per-phase NDT $\delta_1(\mu)=\delta_{\text{MAN}}(\mu)$.} 
		\label{fig:OS_Phase1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.475\textwidth}  
		\centering 
		\vspace{10.5em}
		\begin{tikzpicture}[scale=1]
		\SymModSchemePhaseTwo
		\end{tikzpicture}
		\vspace{-14em}
		\caption{\small Scheme for the second phase ($t\in[T_1+1:T_1+T_2]$) with per-phase NDT $\delta_2(\mu)=\frac{1}{\min\{K,1+\mu M\}}$.}  
		\label{fig:OS_Phase2}       
	\end{subfigure}
	\caption
	{\small Illustration of the proposed one-shot scheme with $M=4$ RNs, $K=2$ UEs and $\mu M=2$ for the worst-case demand scenario. On the one hand, in each channel use of the first phase [cf. (a)], the MAN scheme is used on the SISO DeNB-RN broadcast channel to convey desired symbols of (any combination of) $1+\mu M$ RNs. In the worst-case scenario, where UEs request other files, these symbols represent interference which are zero-forced through cooperative DeNB-RN interference cancelation at (any combination) of $\min\{K,\mu M\}$ UEs. Simultaneously, the scheme exploits RN caches by providing the same UEs with their desired symbols. After $T_1$ channel uses, of the first phase, the demand of the RNs is satisfied. On the other hand, the second phase [cf. (b)] is devoted to communicate, if necessary, the remaining file symbols of the UEs by applying cooperative DeNB-RN zero-forcing beamforming.} 
	\label{fig:OS_Scheme}
\end{figure*} 

\alert{The delivery time of the proposed one-shot is devoted to both RNs and UEs. It is intuitive to expect cases where the delivery of requested files by the UEs may take longer than the delivery of uncached file fractions by the RNs. For instance, we expect that for $M\ll K$, irrespective of the fractional cache size, the file delivery to UEs represents the bottleneck from a delivery time perspective. However, finding the exact areas (including the transition) as a function of $\mu, K$ and $M$ where either RN or UE file delivery represents the bottleneck from a latency perspective for one-shot schemes is of interest. To this end, we conclude from Theorem \ref{th:one_shot_ach_NDT} that the functional behavior of the achievable one-shot NDT changes for different region triplets $(\mu,K,M)$ as follows.} Specifically, when neglecting the discretization of the fractional cache size $\mu$ to values  $\{0,\nicefrac{1}{M},\nicefrac{2}{M},\nicefrac{3}{M},\ldots,\nicefrac{(M-1)}{M},1\}$, Table \ref{tab:def_reg_ach_NDT} specifies how the one-shot NDT expression \eqref{eq:NDT_OS_ach} simplifies for the given region triplets. %\vspace{0.5em}
%\begin{table}
\begin{center}
	\begin{tabular}{ |l|l|c|c|l|}
		\hline
		\multirow{2}{*}{Region Name} & \multirow{2}{*}{Definition} & \multicolumn{2}{c|}{Bottleneck} & \multirow{2}{*}{Achievable NDT} \\\cline{3-4} & & RN side & UE side &  \\ \hline  \multirow{2}{*}{Region A} & $K\leq\mu M<M<\frac{1}{1-2\mu},\mu\leq\frac{1}{2}$ & \multirow{2}{*}{--} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{$\delta_{\text{OS}}^{(\text{A})}(\mu)=1$} \\\cline{2-2}  & $K\leq\mu M\leq M,M>\frac{1}{1-2\mu},\mu>\frac{1}{2}$ & & & \\ \hline
		Region B & $K\leq\mu M,\frac{1}{1-2\mu}\leq M,\mu\leq\frac{1}{2}$ & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} & \multirow{2}{*}{$\delta_{\text{OS}}^{(\text{B,E})}(\mu)=\delta_{\text{MAN}}(\mu)$} \\ \cline{1-2} Region E & $\mu M <K\leq\mu M\cdot\delta_{\text{MAN}}(\mu)\leq M$ & & & \\ \hline
		Region C & $\mu M<M<K$ & \multirow{2}{*}{--} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{$	\delta_{\text{OS}}^{(\text{C,D})}(\mu)=\frac{K+\delta_{\text{MAN}}(\mu)}{1+\mu M}$} \\ \cline{1-2} Region D & $\mu M\cdot\max\Big\{1,\delta_{\text{MAN}}(\mu)\Big\}<K\leq M$ & & & \\ \hline
	\end{tabular}
	\captionof{table}{\small \alert{Definition of $(\mu,K,M)$ region triplets and their achievable one-shot NDT. The achievable one-shot NDT in Region A coincides with the lower bound and is thus NDT-optimal.}}
	%\caption{}
	\label{tab:def_reg_ach_NDT}
\end{center}
%\end{table}

%\begin{itemize}
%	\item $\text{Region A}:\begin{cases}
%	K\leq\mu M<M<\frac{1}{1-2\mu},\mu\leq\frac{1}{2}&(\text{Region A}_1)\\
%	K\leq\mu M\leq M,M>\frac{1}{1-2\mu},\mu>\frac{1}{2}&(\text{Region A}_2)
%	\end{cases}\quad\qquad\qquad\text{ with NDT}$ 
%	\begin{align}\label{eq:ach_OS_NDT_RegA}
%	\delta_{\text{OS}}^{(\text{A})}(\mu)=1,
%	\end{align}
%	\item $\text{Region Pair (B,E)}:\begin{cases}
%	K\leq\mu M,\frac{1}{1-2\mu}\leq M,\mu\leq\frac{1}{2}&(\text{Region B})\\\mu M <K\leq\mu M\cdot\delta_{\text{MAN}}(\mu)\leq M&(\text{Region E})
%	\end{cases}\qquad\text{ with NDT}$
%	\begin{align}\label{eq:ach_OS_NDT_RegBE}
%	\delta_{\text{OS}}^{(\text{B,E})}(\mu)=\delta_{\text{MAN}}(\mu),
%	\end{align}
%	\item $\text{Region Pair (C,D)}:\begin{cases}
%	\mu M<M<K&(\text{Region C})\\\mu M\cdot\max\Big\{1,\delta_{\text{MAN}}(\mu)\Big\}<K\leq M&(\text{Region D})
%	\end{cases}\quad\text{ with NDT}$
%	\begin{align}\label{eq:ach_OS_NDT_RegCD}
%	\delta_{\text{OS}}^{(\text{C,D})}(\mu)=\frac{K+\delta_{\text{MAN}}(\mu)}{1+\mu M}.
%	\end{align}
%\end{itemize}
\begin{figure}
	\centering
	\begin{tikzpicture}[scale=1]
	\PlotMMuRegionsTwo
	\end{tikzpicture}
	\caption[Plot of all regions]{\small 2D $(\mu,M)$-plot of all Regions A, B, C, D and E for constant $K$ $(K=2)$. The labels on the graph indicate the functional relationship at the borders of neighboring regions. The discrete points illustrate the fractional cache sizes $\mu\in\Big\{0,\frac{1}{M},\ldots,\frac{M-1}{M},1\Big\}$ for which the achievable one-shot NDT expression $\delta_{\text{OS}}(\mu)$ in Eq. \eqref{eq:NDT_OS_ach} actually hold.}
	\label{fig:Region_plot_advanced}
\end{figure} \alert{The regions of Table \ref{tab:def_reg_ach_NDT} are illustrated in Fig. \ref{fig:Region_plot_advanced} for constant $K$ ($K=2$).} We state two interesting observations on these regions in the following remarks.

\begin{remark}
	Interestingly, when $M\geq 2K+1$, we see that for $\mu\geq\nicefrac{1}{M}$, the achievable one-shot NDT does not depend on $K$, i.e., the number of UEs. Instead, the NDT is solely dependent on the number of RNs $M$. Consequently, our one-shot NDT behaves identical to the achievable NDT of the MAN scheme. This is due to the fact that the bottleneck in the delivery time is governed by the delivery of uncached file fragments to the RNs. Then, this problem reduces to the initial receiver-based, single server coded caching problem of Maddah-Ali and Niesen. For this setting, we recall that the MAN NDT for $M$ receivers consists of the local and global caching gains (captured by the factors $1-\mu$ and $\frac{1}{1+\mu M}$ in $\delta_{\text{MAN}}(\mu)$, respectively) \cite{Maddah-Ali2}. In conclusion, we refer, respectively, to the attainable NDT as the \emph{DeNB-to-RN broadcast bottleneck NDT} and \alert{cases where $M/K>2$ as cases of \emph{relative high RN} quantities (with respect to the number of UEs)}.  
\end{remark}
\begin{remark}
	As opposed to the previous remark, we observe that in the one-shot scheme the UEs function as the bottleneck from a delivery time perspective as long as $M<2K+1$. \alert{We call these instances, all with respect to the number of UEs, as cases of \emph{relative moderate RN} quantities when $1\leq M/K\leq 2$ and \emph{relative low RN} quantities when $M/K<1$.} We then call the attainable NDT of $\frac{K+\delta_{\text{MAN}}(\mu)}{1+\mu M}$ the \emph{UE bottleneck NDT}.    
\end{remark}

In the following four corollaries, we state the relations of the NDT lower bound from Theorem \ref{theorem_lower_bound} and the one-shot scheme upper bound of Theorem \ref{th:one_shot_ach_NDT} of the aforementioned regions for discretized $\mu$.
\begin{corollary}[One-Shot NDT Optimality]\label{corr:OS_NDT_Opt} The one-shot scheme %presented in Section \ref{cha_one_shot} 
	is optimal (i.e., it coincides with the lower bound) \alert{achieving the minimum NDT given by} $\delta^{\star}(\mu)=1$, when the triplet $(\mu,K,M)$ satisfies any of the following conditions:
	\begin{enumerate}
		\item[1a)] $K<M,\mu\geq\frac{K}{M},\mu M\geq \Bigl\lceil{\frac{M-1}{2}}\Bigr\rceil,\mu\leq\frac{1}{2}$; or
		\item[1b)] $K\leq M,\mu\geq\frac{K}{M}$ and $\mu>\frac{1}{2}$.
	\end{enumerate} 
\end{corollary}	
\begin{proof} The proof follows from the fact that all discretized $\mu$ values inside Region A attain an NDT $\delta_{\text{OS}}^{(A)}(\mu)=1$ that matches the lower bound. 
\end{proof}
%\vspace{0.5em}
\begin{remark}
	With this corollary, we make the observation that at \emph{relative high RN} quantities a fractional cache size of \emph{approximately} $\nicefrac{1}{2}$ is sufficient of achieving the lowest attainable NDT of $1$. \alert{In other words, this shows that when $M/K>2$ prefetching half of each file (from the entire library of files) and applying the one-shot scheme is \emph{delivery time optimal}.} Caching more than that will \emph{not} reduce the delivery time any further.         
\end{remark}
The remaining three corollaries state the multiplicative gap of the one-shot scheme with respect to the lower bound. 
%The proofs of these corollaries will be given in multiple subsection of \ref{cha_gap}. 
\vspace{0.5em}
\begin{corollary}[\alert{Gap of NDT for High Relative RN Quantities ($M/K>2$)}]\label{corr:Gap_OS_NDT_High_RN_Quantity} The multiplicative gap between the one-shot scheme presented in Section \ref{cha_one_shot} and the lower bound on the NDT for $M\geq 2K+1$ is \alert{upper bounded by} %within 
	\begin{enumerate}
		\item[1a)] $\frac{M-1}{2}$ for $\mu\leq\frac{1}{M}$,
		\item[1b)] $\frac{M-\theta}{1+\theta}$ for any $\mu\in\Big[\mu'(\theta),\frac{\ceil{\nicefrac{(M-1)}{2}}}{M}\Big]$, where $\mu'(\theta)=\frac{\ceil{\theta}}{M}$ and $\theta\in\Big[1,\frac{M-3}{2}\Big]$.
	\end{enumerate}	
	\begin{proof} \alert{The proof of this corollary is given in Chapter \ref{cha_gap}. Specifically, 1a) is shown in \ref{subsec:de_reg_pair_gap} and 1b) in \ref{subsec:be_reg_pair_gap}.}  
	\end{proof}
\end{corollary}	
\vspace{0.5em}
\begin{corollary}[\alert{Gap of NDT for Moderate Relative RN Quantities ($1\leq M/K\leq 2$)}]\label{corr:Gap_OS_NDT_Moderate_RN_Quantity} The multiplicative gap between the one-shot scheme presented in Section \ref{cha_one_shot} and the lower bound on the NDT at \emph{moderate relative RN quantities} is 
	\begin{enumerate}
		\item $1$ for $K=1$
		and within (or upper bounded by)
		\item[2a)] $\frac{K}{2}+\frac{M-1}{4}$ for $\mu\leq\frac{1}{M}$ and $K\geq 2$,
		\item[2b)] $\frac{dK}{M+1}+\frac{d(d-1)}{M+1}$ for any $\mu\in\Big[\mu'(\kappa_d),\frac{K}{M}\Big]$, where $\mu'(\kappa_d)=\frac{\ceil{\kappa_d}}{M}$, $\kappa_d=\frac{M+1-d}{d}$ and $d\in\Big[\frac{M+1}{K},\frac{M+1}{2}\Big]$ for $K\geq 2$.
	\end{enumerate}	
\end{corollary}
\begin{proof} \alert{The proof of this corollary is given in subsection \ref{subsec:cd_reg_pair_gap} of Chapter \ref{cha_gap}.}  
\end{proof}	
\vspace{0.5em}
\begin{corollary}[\alert{Gap of NDT for Low Relative RN Quantities ($M/K<1$)}]\label{corr:Gap_OS_NDT_Low_RN_Quantity} The multiplicative gap between the one-shot scheme presented in Section \ref{cha_one_shot} and the lower bound on the NDT at \emph{low relative RN quantities} is 
	\begin{enumerate}
		\item $1$ for $(K,M)=(1,2)$
		and upper bounded by 
		\item $1+\frac{1}{K}\Big(\frac{K}{2}-\frac{2}{K}\Big)$ for $M=1,K>2$,
		\item[3a)] $1+\Big(\frac{K}{2}+\frac{M-5}{4}\Big)\cdot\frac{M}{K}\cdot\frac{(K+M+1)}{(K+M-1)}$ for $\mu\leq\frac{1}{M}$ and $M\geq 2$,
		\item[3b)] $d+\frac{d(d-1)}{K}$ for any $\mu\in\Big[\mu'(\kappa_d),1\Big]$, where $\mu'(\kappa_d)=\frac{\ceil{\kappa_d}}{M}$, $\kappa_d=\frac{M+1-d}{d}$ and $d\in\Big[\frac{M+1}{M},\frac{M+1}{2}\Big]$ for $M\geq 2$.
	\end{enumerate}	
\end{corollary}	
\begin{proof} \alert{The proof of this corollary is given in subsection \ref{subsec:cd_reg_pair_gap} of Chapter \ref{cha_gap}.}  
\end{proof}	
We use the last three corollaries to show that a fractional cache size of approximately $\nicefrac{1}{2}$ generates a \emph{constant} multiplicative gap less than $3$ for arbitrary $K$ and $M$. This is stated in the following corollary. 

\begin{corollary}[Constant Gap]\label{corr:const_gap} For fractional cache sizes $\mu\geq\mu_{C}\triangleq\frac{\ceil{\nicefrac{(M-1)}{2}}}{M}$ the multiplicative gap between the one-shot scheme presented in Section \ref{cha_one_shot} and the optimal NDT is constant \alert{versus $\mu$} and is \alert{bounded by %within 
		a factor of $\nicefrac{8}{3}$.} 
\end{corollary}	  
\begin{proof}
	At high relative RN quantities, the NDT optimality at $\mu_{C}$ is shown in Corollary \ref{corr:OS_NDT_Opt}. For this case, the gap is per definition of optimality $1$. \alert{Next, at moderate RN quantities, the gap is, respectively, for $K=1$ and $(K,M)=(2,2)$ $1$ and $\frac{5}{4}$ as stated by Corollary \ref{corr:Gap_OS_NDT_Moderate_RN_Quantity} (points 1 and 2b) with $d=\frac{3}{2}$). Also at moderate relative RN quantities, when $K\geq2, M\geq 3$, we use point 2b) with $d=2$ to find the multiplicative gap} 
	\begin{align*}
	\frac{dK}{M+1}+\frac{d(d-1)}{M+1}\Bigg|_{d=2}=\frac{2(K+1)}{M+1}\leq 2
	\end{align*} for fractional cache sizes $\mu\geq\mu'(\kappa_2)=\mu_C=\frac{\ceil{\nicefrac{(M-1)}{2}}}{M}$. Finally, at low relative RN quantities, the gap for the special cases $(K,M)=(2,1)$ and $M=1,K>2$ are according to 1) and 2) of Corollary \ref{corr:Gap_OS_NDT_Low_RN_Quantity} $1$ and
	\begin{align*}
	1+\frac{1}{K}\Big(\frac{K}{2}-\frac{2}{K}\Big)\leq\frac{3}{2},
	\end{align*} respectively. Additionally, when $M\geq 3$, 2b) of Corollary \ref{corr:Gap_OS_NDT_Low_RN_Quantity} with $d=2$ generates the gap \begin{align*}
	d+\frac{d(d-1)}{K}\Bigg|_{d=2}=2\bigg(1+\frac{1}{K}\bigg)\leq2\bigg(1+\frac{1}{M}\bigg)\leq\frac{8}{3}.
	\end{align*} Combining all cases, we conclude that the gap is bounded from above by $\nicefrac{8}{3}$.   
\end{proof} In conclusion, this corollary shows that one-shot schemes at fractional cache sizes of $\frac{1}{2}$ $\Big(\frac{1}{2}\geq\frac{\ceil{\nicefrac{(M-1)}{2}}}{M}\Big)$ are optimal within a constant \alert{(with respect to the lower bound) multiple gap of optimality}. 
%These schemes, apart from the full-duplex capabilities of the RNs, are simpler in implementation and thus practically more applicable than alignment schemes presented in Section \ref{sec:ach_special}.
\alert{The main disadvantage of this scheme becomes visible when considering regions C and D. For these regions, the first and second phase provide (per channel use) only a subset of $\mu M$ and $\min\{K,1+\mu M\}$ UEs with their desired symbols while the remaining UEs observe interference. Interference alignment provides the opportunity of alleviating the effect of undesired symbols. To this end, we establish achievability schemes that involve a novel beamforming design that facilitates (i) multicasting opportunities (when $M\geq 2$) on the DeNB-RN broadcast channel, (ii) (joint) zero-forcing opportunities and (iii) subspace interference alignment. The notion of subspace alignment was first introduced in \cite{Suh08}. The idea is to align interferences into a multi-dimensional subspace instead of a single dimension \cite{MaddahAliAlignment}. Through this beamforming design, we were able to establish the complete NDT-tradeoff for $K+M\leq 4$. The following theorem specifies this tradeoff.}   
\begin{theorem}[Optimal NDT Tradeoff]\label{th:opt_NDT_tradeoff}
	The optimal NDT tradeoff for the transceiver cache-aided network with one DeNB, $M$ RNs each endowed with a cache of fractional cache size $\mu\in[0,1]$, $K$ UEs satisfying $K+M\leq 4$ with $N\geq K+M$ \alert{number of files}, is given as 
%\begin{align}\label{eq:NDT_opt_trade_off}
%\delta^{\star}(\mu)=\max\Bigg\{&1,K+M-\mu M(K+M-1),\frac{K+M-\mu\Big(M^2+(K-3)(M-1)\Big)}{2},\nonumber\\&\qquad\frac{K+M-1-\mu\Big((M-1)(K+M-3)\Big)}{2}\Bigg\}.
%\end{align}
\begin{align}\label{eq:NDT_opt_trade_off}
\delta^{\star}(\mu)=\max\Bigg\{&1,K+M-\mu M(K+M-1),\frac{K+M-\mu\Big(M^2+(K-3)(M-1)\Big)}{2},\nonumber\\&\qquad\frac{K+M-1-\mu\Big(\alert{M^{2}+(K-3)(M-1)+3}\Big)}{2}\Bigg\}.
\end{align}
\end{theorem}
\begin{proof}
The lower bound on the NDT for this setting readily follows from Theorem \ref{theorem_lower_bound}. Concretely, the last three terms inside the max-expression of \eqref{eq:NDT_opt_trade_off} correspond to %$\delta_{\text{LB}}(\mu,\ell=M,s=1)$, $\delta_{\text{LB}}(\mu,\ell=M,s=2)$ and $\delta_{\text{LB}}(\mu,\ell=M-1,s=1)$
\alert{$\delta_{\text{LB}}(\mu,M,1)$, $\delta_{\text{LB}}(\mu,M,2)$ and $\delta_{\text{LB}}(\mu,M-1,1)$}, respectively. The outer bound (achievability) on the NDT is presented in Section \ref{sec:ach_special}. Shortly, we establish the achievability for (at most) four corner points at \alert{zero-cache and full-cache} fractional cache sizes $\mu=0$, $\mu=1$ as well as \alert{intermediate} cache sizes $\mu'$ in the interval $0<\mu'<1$. The first two corner points are achievable through DeNB broadcasting and cooperative DeNB-RN zero-forcing beamforming (cf. Lemma \ref{corr_mu_0_and_1}). \alert{In the achievability scheme at intermediate fractional cache size $\mu=\nicefrac{K}{M}$, on the other hand, the one-shot scheme of Theorem \ref{th:one_shot_ach_NDT} is optimal for $(K,M)\in\{(1,2),(2,2),(1,3)\}$. For the cases $(K,M)\in\{(3,1),(2,2)\}$, respectively, we establish the optimal NDT at fractional cache sizes $\nicefrac{4}{5}$ and $\nicefrac{4}{9}$ through optimized precoding design that synergistically combines subspace alignment and MAN multicasting with zero-forcing beamforming consuming \emph{finite} channel uses.}     
\end{proof}






==> tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
      \pgf@temp
      \fi%
    },
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
        \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{\csname pgfk@/tikz/tikzmark prefix\endcsname#1\csname pgfk@/tikz/tikzmark suffix\endcsname}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname{\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
      \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
      \pgfsys@getposition{\pgfpictureid}\save@this@pic%
      \pgf@process{\pgfpointorigin\save@this@pic}%
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
      \pgf@process{\pgfpointorigin\save@orig@pic}%
      \advance\pgf@x by -\pgf@xa
      \advance\pgf@y by -\pgf@ya
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
          \advance \pgf@xa by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@x\relax
\advance \pgf@ya by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@y\relax
          \advance \pgf@xa by -\csname save@pg@\pgfpictureid\endcsname\pgf@x\relax
\advance \pgf@ya by -\csname save@pg@\pgfpictureid\endcsname\pgf@y\relax
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }
\begingroup
\catcode`\;=\active
\gdef\tikzmark@active#1#2{%
\tikz[remember picture with id=#2] #1;}
\endgroup
\def\tikzmark@nonactive#1#2{%
\tikz[remember picture with id=#2] #1;}
\newcommand\tikzmark@outside[2][]{%
  \ifnum\catcode`\;=\active
   \let\tikzmark@next=\tikzmark@active
  \else
   \let\tikzmark@next=\tikzmark@nonactive
  \fi
  \tikzmark@next{#1}{#2}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x pt}{\the\pgf@y pt}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark}[2][]{\only#3{\beameroriginal{\tikzmark}[{#1}]{#2}}}
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@#1}{%
      #3%
    }{%
      #2%
    }%
  }%
\newcommand\subnode[3][]{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@shape{rectangle}%
  \def\tikz@anchor{center}%
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
  {\PackageError{pgf}{Unknown shape ``\tikz@shape''}{}}%
  {%
    {%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \def\pgf@sm@shape@name{\tikz@shape}% CJ % TT added prefix!
      \csname pgf@sh@s@\tikz@shape\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
       \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}% FIXME : this is double work!
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@node@name{\tikz@fig@name}%
      \ifx\pgf@node@name\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{\tikz@shape}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp
        \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
      \fi%
    }%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}
\def\usetikzmarklibrary{\pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}}%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

%% 
%% Copyright (C) 2011-2016 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.

